Reverse Psychology in Trust-Aware Human-Robot Interaction

To facilitate effective human-robot interaction (HRI), trust-aware HRI has been proposed, wherein the robotic agent explicitly considers the human's trust during its planning and decision making. The success of trust-aware HRI depends on the specification of a trust dynamics model and a trust-behavior model. In this study, we proposed one novel trust-behavior model, namely the reverse psychology model, and compared it against the commonly used disuse model. We examined how the two models affect the robot's optimal policy and the human-robot team performance. Results indicate that the robot will deliberately "manipulate" the human's trust under the reverse psychology model. To correct this "manipulative" behavior, we proposed a trust-seeking reward function that facilitates trust establishment without significantly sacrificing the team performance.

==> RA-L_ICRA 2021 HRI simulation/0Abstract.tex <==
\begin{abstract}
To facilitate effective human-robot interaction (HRI), trust-aware HRI has been proposed, wherein the robotic agent explicitly considers the human's trust during its planning and decision making. The success of trust-aware HRI depends on the specification of a trust dynamics model and a trust-behavior model. In this study, we proposed one novel trust-behavior model, namely the reverse psychology model, and compared it against the commonly used disuse model. We examined how the two models affect the robot's optimal policy and the human-robot team performance. Results indicate that the robot will deliberately \textcolor{black}{``manipulate''} the human's trust under the reverse psychology model. To correct this ``manipulative'' behavior, we proposed a trust-seeking reward function that facilitates trust establishment without significantly sacrificing the team performance. 
% We found that under certain conditions, a Nash equilibrium occurs when both the human and the robot assume the disuse model.
\end{abstract}


==> RA-L_ICRA 2021 HRI simulation/1Sections.tex <==
\section{Introduction}\label{sec:intro}

Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve every sector of our economy and improve how people live and work. However, realizing the full potential of these technologies is only possible if people establish appropriate trust in them \cite{Sheridan:2016kn, Azevedo_context, Yang:2017:EEU:2909824.3020230, du2020not}.

% Trust has been identified as one central factor for effective human-robot interaction (HRI) and has received a substantial amount of research attention 

% Existing work on trust in human-robot interaction (HRI) can be broadly classified into two bodies of research. The first line of research originated from psychology/human factors, wherein trust is measured using questionnaires. Using the questionnaire approach, more than two dozen factors have been identified to influence trust in human-robot interaction, including individual factors such as culture and age~\cite{Rau2009}, system factors such as reliability~\cite{Salem2015}, and environmental factors such as task emergency~\cite{Robinette:2016_HRI}. Other factors related to the physical embodiment of a robot (e.g., anthropomorphism \cite{Kiesler2008}) have also been reported. 

\textcolor{black}{To facilitate effective human-robot interaction (HRI), trust-aware HRI has been proposed, aiming to enable the robot to explicitly consider the human's trust in its decision making process \cite{chen2020trust}. The success of trust-aware HRI depends on two components: the trust dynamics model and the trust-behavior model. A trust dynamics model specifies how a human's trust changes in response to moment-to-moment interaction with a robot \cite{Guo2020_IJSR}. A trust-behavior model describes the human's behavior as a function of trust. Note that trust and behavior are distinct constructs: trust in autonomy is the ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability \cite{See:2004vj}" while behavior is the human's compliance and reliance behavior, which is affected by his or her attitude.}

\textcolor{black}{Active research has been conducted to examine the trust dynamics model. Researchers have proposed computational models for inferring a human's trust in a robotic agent at any time based on the robot's performance, the human's behavioral information, and physiological information \cite{Guo2020_IJSR, xu2015optimo, Lu2020, hu2016real,Azevedo-Sa2020}. Little research, however, has investigated the trust-behavior model. Previous research largely assumed a disuse trust-behavior model~\cite{chen2020trust}, wherein a human will stop relying on a robot when his or her trust in the robot is low. However, psychological research has shown that people may display reverse-psychology behaviors~\cite{macdonald2011people}, which means a human will do exactly the opposite of what the robot suggests.}


% This approach allows researchers to infer (measure) a human's trust toward a robot in real-time and enables the design of trust-aware robots by incorporating trust into the robot's planning and decision making \cite{chen2020trust}. 




% The second body of research originated from computer science/robotics. In this line, trust is considered a variable internal to a human but can be inferred using other observable information. 

% ``Humans' trust in automation, or more recently trust in autonomy, has received extensive research attention in the past three decades. The diverse interest has generated multiple definitions including trust as a belief, an attitude, and a behavior [6]. In this paper, we use the definition by Lee and See [8]: Trust is the ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (Please see [6,9,10] for more discussion on the definitions of trust in automation and see [11-13] for examples using the Lee and See's definition).”




% Our contributions are summarized as follows. We propose two novel trust-behavior models, i.e., the disuse model and the reverse psychology model. In the disuse model, when a human's trust is below a certain threshold, s/he will completely ignore the robot and use his or her own policy; In the reverse psychology model, the human will do the opposite of what the robot recommends when his or her trust is below a threshold. 


In this study, we simulate and compare how the disuse and the reverse psychology models affect trust-aware decision making and the human-robot team's performance. Results indicate that the robot will display certain ``manipulative'' behavior 
% if the human's trust at low-trust states 
if it assumes the human uses the reverse psychology model. Although this ``manipulative'' behavior may seem beneficial to the task performance in a short term, it could eventually undermine the human-robot interaction in the long run, e.g., leading to the disuse of the robot. To overcome such \textcolor{black}{``manipulative''} behaviors, we propose a trust-seeking reward function to prevent the robot from actively guiding the human to reduce his or her trust in order to take advantage of the reverse psychology behavior. We suggest augmenting a reward for gaining the human's trust in the short term, which will result in large benefits in the long run. 
% We also find that under certain conditions, a Nash equilibrium occurs when both parties assume the disuse model. To the best of our knowledge, our study is the first attempt to study the trust-behavior models in computational settings, which paves the way for many future studies and applications.

The rest of the paper is organized as follows: Section~\ref{sec:relatedWork} reviews related work in trust-driven human-robot interaction; Section~\ref{sec:model} formulates the trust-aware decision making problem in a POMDP framework and describes the trust-behavior model as well as the trust-seeking reward function;  Section~\ref{sec:case} introduces a reconnaissance mission as a study case to examine how different settings affect the interaction; Section~\ref{sec:result} reports the simulation results and our observations; Section~\ref{sec:discussion} summarizes our findings and discussed the limitations and future directions of this study. 

% \vfill

%===================================================
%===================================================
\section{Related Work}\label{sec:relatedWork}

To enable trust-aware HRI, a robot should be able to estimate a human's trust based on the interaction history, anticipate how trust influences their interaction, and consequently choose the optimal action that maximizes a given goal. These three steps correspond to three major components in trust-aware HRI, i.e., trust dynamics, a trust-behavior model, and a trust-aware decision-making framework. We review them in the rest of this section.


\subsection{Trust Dynamics Model}


To model trust dynamics and predict a human's trust in real time, prior work has proposed several trust estimators. Lee and Moray~\cite{Lee:1992it} proposed the auto-regressive moving average vector (ARMAV) model calculating trust as a function of task performance and the occurrence of automation failures. Xu and Dudek~\cite{xu2015optimo} built the online probabilistic trust inference model (OPTIMo) based on the dynamic Bayesian network framework, treating the human's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human's behavior. Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human's electroencephalography (EEG) and galvanic skin response (GSR) data. Lu and Sarter~\cite{Lu2020} used three machine learning techniques, namely, logistic regression, k-Nearest Neighbors (kNN), and random forest, to classify the human's real-time trust level using eye-tracking metrics. More recently, Soh et al.~\cite{soh2020multi} proposed a Bayesian Gaussian Process trust model, assuming the human trust evolves via Bayes rule and placing a Gaussian process prior over the trust function. In this work, we use the trust model proposed by Guo and Yang~\cite{Guo2020_IJSR}, where trust is modeled as a Beta distribution characterized by positive and negative interaction experiences. This Beta distribution model adheres to three important properties of trust dynamics \cite{Yang:2021}, namely, \textit{continuity}, \textit{negativity bias}, and \textit{stabilization}, thus providing good model predictability, explicablity, and generalizability. 



% Guo and Yang~\cite{Guo2020_IJSR} modeled trust as a Beta distribution characterized by positive and negative interaction experiences. The Beta distribution model adheres to important properties of trust dynamics reported in empirical studies, thus providing good model predictability, explicablity, and generalizability. 



\subsection{Trust-behavior Model}
Trust-behavior models aim to predict human's compliance and reliance behaviors as a function of trust. Although the research in psychology/human factors does not focus on developing a mathematical model, the general conclusion is that the more a human trusts a robot, the more likely s/he will use the robot or accept the robot's recommendation. As a result, in computational HRI studies, a mathematical trust-behavior model is usually characterized by a simple function. For example, Chen et al.~\cite{chen2020trust} modeled the probability of a human using a robot as a sigmoid function of trust.

Our study considers two possible trust-behavior models, namely the disuse model and the reverse psychology model. The distinction between the two models lies in the different behaviors when a human's trust is low. In the disuse model, the human will completely ignore the robot's recommendations and only follow his or her own decision; In the reverse psychology model, the human will do the opposite (i.e., If a robot recommends going east, the human will go west). The use of reverse psychology has been reported in human-human interaction~\cite{macdonald2011people}.


\subsection{Trust-Aware Decision Making in HRI}
With a trust dynamics model and a trust-behavior model, a robot can predict how a human's trust will change due to moment-to-moment interactions and how the human's behavior will change as a function of trust, and in turn to plan its actions accordingly. Existing studies in trust-aware decision-making is formulated based on the Markov decision process (MDP) framework. Chen et al.~\cite{chen2020trust} proposed the trust-POMDP to let a robot actively calibrate its human teammate's trust. Their human-subject study showed that purely maximizing trust in a human-robot team may not improve team performance. Losey and Sadigh~\cite{losey2019robots} modeled human-robot interaction as a two-player POMDP where the human does not know the robot's objective. They proposed 4 ways for the robot to formulate the human's perception of the robot's objective and showed the robot will be more communicative if it assumes the human trusts itself and thus increase the human's involvement.


%===================================================
%===================================================
\section{Mathematical Model}\label{sec:model}


\subsection{General Framework}
We formulate the trust-aware HRI as a compact POMDP $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is the set of interaction states, $A$ is the set of robot's action, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $\Omega $ is the set of observations, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is the reward function specifying the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The robot runs the POMDP model during the interaction as follows: At time $k$, the robot holds belief $b_k$ over the state of the system $s_k$ and then takes action $a_r=\pi_r(b_k)$, where $\pi_r: B \rightarrow A$ is a policy mapping from the belief state space $B$ to action space $A$. This action $a_r$ takes $s_k$ to the next state $s_{k+1}$ via the transition function $T$ and generate an observation $o_k$ and a reward $r_k$. Then the robot updates its belief over $s_{k+1}$ by observing $o_k$ and goes to time $k+1$. The goal of running this POMDP is to solve the optimal policy $\pi^*$ to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{N}_{k=1} \gamma ^{k} r_{k}\right]$. The transition function $T$ and the observation function $O$ are based on the interaction context. Particularly, in this study, they are determined by the environment model, the trust dynamics model, and the trust-behavior model. 


We exploit the performance-induced trust model ~\cite{Guo2020_IJSR, Yang:2021} to predict a human's trust. Trust $t_k$ before the $k$th interaction is defined as a random variable given by a Beta distribution
\begin{equation}
\label{eq:BetaTrust}
    t_{k} \sim \mathbf{Beta}(\alpha _{k} ,\beta _{k} )
\end{equation}
and the two positive shape parameters $\alpha _{k}$ and $\beta _{k}$ are updated by
\begin{equation}
\ ( \alpha _{k} ,\beta _{k}) =\begin{cases}
\left( \alpha _{k-1} +w^{s} ,\beta _{k-1}\right) &\text{ if } \ p_{k} =0,\\
\left( \alpha _{k-1} ,\beta _{k-1} +w^{f}\right) &\text{ if } \ p_{k} =1.
\end{cases}
\label{eq:trust_update}
\end{equation}
where $p_{k}$ is the performance of the robot on the $k$th task defined as a binary variable on $\{0,1\}$; $\alpha _{k}$ and $\beta _{k}$ are the cumulative negative and positive interaction experience respectively so far; and $w^{s}$ and $w^{f}$ are the experience gains due to the robot's success and failure at each task. As a consequence, the experience tuple $(\alpha_k,\beta_k)$ is a sufficient statistics to describe trust history, because given $(\alpha_k,\beta_k)$, how future trust evolves does not depend on the interactions earlier than the $k$th one. As a result, we can use $(\alpha_k,\beta_k)$ to denote the belief over trust $t_k$.


\subsection{Two Trust-Behavior Models}
We propose two trust-behavior models. The human's behavior model is a function $\pi_b(a_h, I)=p( a_h|I)$ assigning a probability to each of the human's actions $a_h$ given his or her own knowledge $I$. Because the probability of a human accepting the recommendation of a robot is highly related to the human-robot trust~\cite{See:2004vj}, we model that the probability of the human accepting the robot's recommendation is determined by trust, i.e., $p( a_h{=}a_r|I)=\varphi (\frac{\alpha }{\alpha +\beta })$, \textcolor{black}{where $\varphi$ is non-decreasing}. To specify the human's behavior when s/he is \emph{not} following the recommendation, we consider two possible trust-behavior models, namely, the reverse psychology model and the disuse model, as shown in  Figure~\ref{fig:behaviors}. 

\textbf{Reverse psychology model.} The first model is termed the \emph{reverse psychology} model $\pi_b^r$. When trust is high, the human will follow the robot's recommendation with a high probability. However, when the human-robot trust is low, the human will tend to do the \emph{opposite} to what the robot says. More precisely, by letting $\bar{\varphi} := 1 - \varphi$, we have
\begin{equation}
\pi_b^r(a_h,I) =\begin{cases}
\varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \textcolor{black}{\text{if following recommendation},}\\
\bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right) & \textcolor{black}{\text{else doing the opposite.}}
\end{cases}
\label{eq:reverseModel}
\end{equation}

\textbf{Disuse model.} The second model is termed the \emph{disuse} model $\pi_b^d$. When trust is high, the human will follow the robot's recommendation with a high probability. When trust is low, the human will probably ignore the robot's recommendation and follow his or her own policy. More precisely,
\begin{equation}
\pi_b^d(a_h,I) =\begin{cases}
\varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \ \textcolor{black}{\text{if following recommendation},}\\
\bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right) & \ \text{else exercising own policy.} 
\end{cases}
\end{equation}


\begin{figure}[h]
  \centering
  \includegraphics[width=0.9\linewidth]{fig/behaviorModels.pdf}
  \caption{Two trust-behavior models. On one hand, the human will be more likely to follow the robot's recommendation when trust is high. On the other hand, when trust is low, the human will take the opposite recommendation in the reverse psychology model while exercise his or her own policy in the disuse model.}
  \label{fig:behaviors}
\end{figure}

\subsection{Reward Function}
The reward function is determined by the specific task the human-robot team works on. We denote this task-induced reward function as $R_m$. The goal of the team is to maximize the total mission reward $J=\mathbb{E}\left[\sum ^{N}_{k=1} \gamma ^{k} R_m(k)\right]$. Later in the simulation, we show if the robot only plans to maximize the task reward $R_m$, it will deliberately \emph{manipulate} the human in the reverse psychology model. That is, the robot may deliberately make an opposite recommendation when the human's trust is low (so as to maximize potential reward). This is a result of the absence of trust in the task reward. However, purely maximizing human-trust would harm task performance~\cite{chen2020trust}. To correct this \textcolor{black}{``manipulative''} behavior while \textcolor{black}{letting} the robot focus on the task reward, we propose a trust-seeking reward function
\begin{equation}
\label{trust-seeking}
    R_t(k)=R_m(k) + \lambda(k)\mathds{1}(\mathcal{A}_k),
\end{equation}
where $\mathcal{A}_k$ is the event when the robot's action leads to trust gain, and $\lambda(k)$ is a positive weight and decreases when $k$ increases. The extra term $\lambda(k)\mathds{1}(\mathcal{A}_k)$ will force the robot to gain trust in near sites and optimize the mission reward in the long run.


\subsection{Value Function and Action Function of POMDP}\label{sec:valActFunctions}
The value function and action function are crucial tools for analyzing a POMDP. We describe them here for later use. The value function $V_{k}(b)$ is defined as the optimal expected cumulative reward starting from belief $b$ at time $k$. And it satisfies the Bellman equation 
\begin{equation}
V_{k}(b) =\max_{a}\mathbb{E}\left[ R(b,a) +\gamma \sum _{b'} P( b'\ |\ b,a) V_{k+1}( b')\right].
\end{equation}
The action function $A_{k}(b)$ is defined as the action to take to achieve $V_{k}(b)$ starting from state $b$ at time $k$, i.e.,
\begin{equation}
A_{k}(b) =\arg \max_{a}\mathbb{E}\left[ R(b,a) +\gamma \sum _{b'} P( b'\ |\ b,a) V_{k+1}( b')\right].
\end{equation}



\section{Case Study}\label{sec:case}
To investigate how different trust-behavior models and different reward functions influence the robot's optimal policy, we use a reconnaissance mission wherein a human teams up with a robot to search several sites in a town for potential threats. The scenario is motivated by~\cite{wang2016impact}. At each site, the robot enters initially, scanning for potential threats, and then recommends to the human if s/he should wear protective gear before entering the site. The protective gear is heavy and wearing it is time-consuming. If the human wears the protective gear and enters a site but finds no threat, the human-robot team wastes precious time; Conversely, if the human decides not to wear the protective gear, s/he will be harmed if a threat is present. The goal of the human-robot team is to complete the mission as soon as possible while minimizing the human's health loss.

Assume the human-robot team is going to search $N$ sites. At site $k$, the probability $d_k$ of having a threat follows a uniform distribution $\mathbf{U}[0,1]$, and the actual presence of the threat $\eta_k$ follows a Bernoulli distribution $\mathbf{Bern}(d_k)$. The human-robot team does not know $d_k$. Instead, prior to the start of the mission, they are provided with intelligence information, showing $\tilde{d}_k$ as an estimation of $d_k$. Before entering site $k$, the robot will analyze the site based on its sensory input and reach a more accurate estimation $\hat{d}_k$ of $d_k$. $\tilde{d}_k$ and \textcolor{black}{$\hat{d}_k$} follow Beta distribution $\mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))$ and $\mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))$ respectively. We constrain that $\kappa_2 > \kappa_1\geq 1$ to reflect the assumption that the robot assesses $d_k$ more accurately than the intelligence information given prior to the mission. Therefore, we have the following relation:
\begin{equation}
\label{eq:threatLevel}
    \begin{split}
        \eta_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Bern}(d_k)\\
        d_k & \overset{\text{i.i.d.}}{\sim} \mathbf{U}[0,1]\\
        \tilde{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))\\
        \hat{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))
    \end{split}
\end{equation}

The state space $S=\{t \ | \ t\in [0,1]\}$ is set of all possible value of trust. $t_k$ is the human's trust before searching the $k$th site and follows the beta distribution $\mathbf{Beta}(\alpha_k,\beta_k)$ as in Eq.~\eqref{eq:BetaTrust}. Consequently, we define the corresponding belief state as $b_k=(\alpha_k,\beta_k)$. The initial belief state is $b_1=(\alpha_1,\beta_1)$ . The robot's action set is $A=\{a_r\ |\ a_r\in \{0,1\}\}$, where $a_r=1$ and $a_r=0$ stand for recommending wearing and not wearing the protective gear respectively. The observation set is the human's perceived performance $p$ of the robot $\Omega=\{p\ |\ p\in\{0,1\}\}$. The observation function $O$ specifies the value of $p$: if robot's recommendation agrees with the presence of the threat then $p=1$,  otherwise $p=0$. For instance, if robot recommends to wear the gear and there does exist a threat in the site, then $p=1$. The transition function $T$ updates each state $(\alpha_k,\beta_k)$ according to Eq.~\eqref{eq:trust_update}. 


Denote the human action as $a_h$, where $a_h=1$ when the human decides to wear the gear while $a_h=0$ otherwise. If the human follows the reverse psychology trust-behavior model $\pi_b^r$, then $a_h$ is given by Eq.~\eqref{eq:reverseModel}, i.e., $a_h=a_r$ with probability $\varphi\left({\alpha }/{\alpha +\beta }\right)$ and $a_h\neq a_r$ with probability $\bar{\varphi}\left({\alpha }/{\alpha +\beta }\right)$. If the human follows the disuse model $\pi_b^d$, then with probability $\bar{\varphi}\left({\alpha }/{\alpha +\beta }\right)$, s/he will ignore the robot and \textcolor{black}{exercise} self-judgement. The information available for him to estimate $d_k$ is the reported danger level $\tilde{d}_k$, so we model that the probability of $a_h=1$ is $\tilde{d}_k$ while it of $a_h=0$ is $1-\tilde{d}_k$. Thus
\begin{equation}
\label{eq:actionDisuse}
\pi_b^d(a_h,I | \text{disusing}) =\begin{cases}
\tilde{d}_{k} &  \text{$a_h=1$}, \ \\
 1-\tilde{d}_{k} &  \text{$a_h=0$}. 
\end{cases}
\end{equation}
In addition, to simplify the simulation and increase the interpretability of the result, we specify $\varphi(\alpha/(\alpha+\beta)) = \alpha/(\alpha+\beta)$. 

The goal of the mission is to complete the task as soon as possible and to minimize the human's health loss. A rational reward function serving this purpose can be \textcolor{black}{a weighted sum of the human's health loss $\delta_h$ (i.e., the human without protective gear will be harmed by a threat) and the time cost $\delta_t$ (i.e., the human-robot team is required to complete the mission as soon as possible) at site $k$. It is given by}
\begin{equation}
\label{eq:threatLevel}
\begin{split}
    &R_m(k)
    =\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right]\\
    =&\sum _{( \delta _{h} ,\delta _{t})}( -w_{h} \delta _{h} -w_{t} \delta _{t}) P\left( \delta _{h} ,\delta _{t} |\tilde{d}_{k} ,\hat{d}_{k} ,\alpha _{k} ,\beta _{k}\right).
\end{split}
\end{equation}
% $R_m(k)$ is the weighted sum of the human's health loss $\delta_h$ (i.e., the human without protective gear will be harmed by a threat) and the time cost $\delta_t$ (i.e., the human-robot team is required to complete the mission as soon as possible) at site $k$. 
% \textcolor{blue}{This reward function is valid because the expected time loss and health loss are determined by the presence of the threat and the human's action, while the latter two variables depend on trust $(\alpha,\beta)$ once $\tilde{d}_k$ and $\hat{d}_k$ are given.}
% Particularly, $R_m(k)$ is determined by the transition function $T$, and the human's behavior model $\pi_b$. 
\textcolor{black}{This reward function is legitimate because the probability $P\left( \delta _{h} ,\delta _{t} |\tilde{d}_{k} ,\hat{d}_{k} ,\alpha _{k} ,\beta _{k}\right)$ is a function of $\tilde{d}_{k} ,\hat{d}_{k} ,\alpha _{k} ,\beta _{k}$ determined by Eq.~\eqref{eq:reverseModel} or Eq.~\eqref{eq:actionDisuse} and $\tilde{d}_{k} ,\hat{d}_{k}$ are constants after the robot scans the site. The value of $(\delta_h, \delta_t)$ should be specified such that wearing gear and the presence of a threat will increase time cost and health loss respectively. An example is shown in  Table~\ref{tab:weighted_sum}. The optimal action at site $n$ is to maximize the expected cumulative rewards  $J=\sum_{k=n}^N \gamma^{k}R_m(k)$.  We do not explicitly specify the units of $\delta_h$ and $\delta_t$ because changing the units has the same effect as changing the weights $w_h$ and $w_t$.}

\begin{table}[h]
\centering
\caption{Value Table of $(\delta_h, \delta_t)$ }
\label{tab:weighted_sum}
\begin{tabular}{c|c|c|c} 
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{}}  & \multicolumn{2}{c}{Protective gear}  \\ 
\cline{3-4}
\multicolumn{2}{c|}{}                   & Yes        & No                      \\ 
\hline
\multirow{2}{*}{Threat existence} & Yes & $(1,300)$  & $(100,50)$              \\ 
\cline{2-4}
                                  & No  & $(0,250)$  & $(0,30)$                \\
\hline
\end{tabular}
\end{table}

\section{Simulation Results and Discussion}\label{sec:result}


\subsection{Simulation Procedure}\label{sec:procedure}
We simulate the reconnaissance mission by iterating the following steps, starting from $n=1$ until $n=N$: 
\begin{enumerate}
    \item At site $n$, the robot has a belief $b_n=(\alpha_n,\beta_n)$ over the human's trust and detects potential threat $\hat{d}_n$;\label{item:sense}
    \item The robot calculates the optimal action $a_n=A_{n}(b_n)$ by solving a $\hat{N}$-step POMDP, where $\hat{N}=N-n+1$. Meanwhile, the robot will calculate the value function $V_n(\alpha_n,\beta_n)$. We note that, since the robot has not scanned site beyond $n$ so far, it will use $\tilde{d}_k$ to estimate $\tilde{d}_k$ for $k>n$;\label{item:VAfunctions}
    \item The human will make his or her choice to wear or not to wear the gear and then search the site, which will reveal the presence of the threat and the mission reward $R_m(n)$ from this site. The mission reward is updated by $J_m = J_m+R_m(n)$. Here the mission reward $J_m$ is different from the expectation of the discounted reward $J$ in the POMDP. The reward $J$ has a discount factor because it needs to discount the uncertainty of the future, while the reward $J_m$ sum up the actual reward collected during the mission;\label{item:soldierBehavior}
    \item The robot will update its belief to $b_{n+1}$ and the team will go to site $n+1$. The process goes to the first step and repeats until reaching the last site.
\end{enumerate}

\subsection{Simulation Experiment 1: Comparing Optimal Policies}
In the first simulation experiment, we examine the robot's optimal policies under different conditions. Particularly, we analyze the policies by inspecting the POMDP's action functions $A_n$ and value functions $V_n$ at each site. 

\textbf{Simulation conditions.} To solve for the robot's optimal policy, we only need to run Steps 1) and 2) described in the simulation procedure, Sec~\ref{sec:procedure}. There are two independent variables in this experiment. The first variable is the robot-assumed trust-behavior model. Because the human's behavior model $\tilde{\pi}_b$ is unknown to the robot, the robot will make certain assumptions on $\tilde{\pi}_b$. We denote $\hat{\pi}_b$ as the robot-assumed trust-behavior model of $\tilde{\pi}_b$. We consider two levels in $\hat{\pi}_b$, i.e., the reverse psychology model ${\pi}_b^r$ and the disuse model ${\pi}_b^d$. The second variable is the reward function $R$, which also has two levels, namely, the task reward $R_m$ and the trust-seeking reward $R_t$.  




\input{big_whole_page_figure}

\afterpage{\clearpage}



\textbf{Model parameters setting.} 
% The parameter setting is shown in Tab.~\ref{tab:exp1Parameters}.
We set the number of total sites $N$ as 15, the value of the health loss $\delta_h$ and time cost $\delta_t$ under different conditions as the ones in Table~\ref{tab:weighted_sum}, the reward weights as $w_h=1$ and $w_t=0.2$, discount factor $\gamma = 0.9$. The parameters of the trust dynamics model in Eq.~\eqref{eq:trust_update} are set to  $w^s=10$ and $w^f=20$ to incorporate the fact that a failure of an automation would have more impact on trust than a success of the automation~\cite{Guo2020_IJSR}. We generated $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ by setting $\kappa_1=3$ and $\kappa_2=50$ in Eq.~\eqref{eq:threatLevel}. We let $\lambda(k) = 80/(1+e^{0.5k})$, so $\lambda(k)$ is decreasing with $k$. We set $\mathcal{A}_k$ as the event when the robot's recommendation $a_r$ agrees with the presence of the threat $\eta_k$. To compare the different conditions, we fixed the random seed for generating $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ so they are assigned the same values across different setups. We used the value iteration method to solve the value functions and action functions.

\textbf{Simulation result.} The simulation result is shown in  Figure~\ref{fig:V_A_functions}. Four sub-figures represent the action functions and value functions of the POMDP under different conditions at 8 selected sites, namely, the site $k=1,3,\cdots,15$. On the top row of each sub-figure are the action functions, while on the bottom row are the value functions. The horizontal axis and the vertical axis are $\alpha_k$ and $\beta_k$, respectively. In each action function, if a state $(\alpha_k,\beta_k)$ is in the black area, then $A_k(\alpha_k,\beta_k)=0$, i.e., the robot's optimal action is to not recommend the human to wear the gear, otherwise $A_k(\alpha_k,\beta_k)=1$, i.e., the robot's optimal action is to recommend the human to wear the gear. In each value function, \textcolor{black}{the brighter} a state $(\alpha_k,\beta_k)$ is, the higher its value $V_k(\alpha_k,\beta_k)$ is. For a better visualization, we use different colormaps for different value functions. So values cannot be compared across different images by the color. 


\textbf{Observation 1: the reverse-psychology model leads the robot to manipulate a human's trust.} The action and value functions in Figure~\ref{fig:a} show the optimal policy demonstrate a \emph{manipulating} behavior under the reverse-psychology-based trust-behavior model and the mission reward. There is a 45-degree line in each action function, across which the optimal action will be reversed. This is a result of the assumption that the human will do the opposite when trust is low. And the shape of this dividing line is determined by the function $\varphi$ in Eq.~\eqref{eq:reverseModel}. Around this line are the neutral trust states where $\varphi(\alpha_k,\beta_k)=0.5$. A decrement of trust in a neutral trust state would result in a future state the human will not follow the robot's recommendation and vice versa. The value functions further reveal that the value of trust is almost symmetric about the 45-degree line. This indicates that, first, a low trust state is equivalent to some high trust state in terms of the reward; second, there is a \emph{strong reinforcement feedback loop} that the robot will actively seek a more untrustworthy status if it is already in an untrustworthy status and vice versa. Moreover, the dividing lines in the action functions except the last one have a small offset towards the trustworthy region. This is a consequence of the fact that the robot's perceived failure has a larger impact on trust compared to the robot's perceived success ($w^f>w^s$). So at a neutral trust state, choosing to manipulate the human will let the robot go faster to a high-value state, i.e., a low-trust state, than choosing the other action. However, at the last site, the robot only needs to act with the human once, so acting either way will obtain the same reward.

\textbf{Observation 2: manipulating behavior is corrected by the trust-seeking reward.} When we modify the reward function to a trust-seeking one by adding a correction term, as described in Eq. \eqref{trust-seeking}, the robot's manipulating behavior can be corrected. In  Figure~\ref{fig:b}, the action function shows that the robot will choose the `righteous' action in most states if it has several rounds of interactions with the human. This happens because the trust-seeking reward encourages the robot to go to a high-trust state even if it is at a neutral state so the robot can collect trust reward in the long run. Consequently, the positive feedback loop near the neutral states is broken and the robot will act righteously even if the initial human-trust is sightly lower than the neutral trust level. Meanwhile, the action function of site 15 indicates the robot will still demonstrate the manipulating behavior if it only needs to interact with the human once. This happens because there are only a few interactions ahead so the robot will primarily focus on the mission reward. Therefore, the trust-seeking term in the reward function can prevent the robot from actively pursuing a low-trust state.

\textbf{Observation 3: the robot will not manipulate the human in the disuse model.}  Figure~\ref{fig:c} shows that the robot will not manipulate the human if it assumes that the human will completely ignore its recommendation. This is a consequence of endowing the human with his or her own reasoning model. Note that trust still plays a role under the disuse assumption since the robot values a high-trust state over a low-trust state, as shown in the value functions. Indeed, because the robot takes its sensed threat level as the ground-truth, it will think the team will get a better mission performance if the human follows its recommendation, i.e., trusting the robot. If we model it reversely by letting the reported threat level be the expected threat level in the POMDP solver, the result shows that the robot would rather let the human use his or her own policy, and thus a low-trust state will have a higher value compared with a high-trust state.

% \vfill

%%%%%%%%%%%%%%%%%%%%%%%%
%%% the big figure %%%%%
%%%%%%%%%%%%%%%%%%%%%%%%


\input{table-experiment2Result}

  
\begin{figure*}[h]
  \centering
  \vspace{4mm}
  \includegraphics[width=\linewidth]{fig/simulationRewardCompareBarWithErrorBar3rd.pdf}
  \caption{The grouped bar-plot of the mean of the team performance $\overline{J}_m$ and the mean of the final trust $\overline{\hat{t}}_N$ in the simulation under different assumptions. Different groups correspond to different values of $\kappa_1$ and $\kappa_2$, the accuracy of the reported threat level and the robot-sensed threat level respectively. Within a group, the bars correspond to different setting on the reward function $R$, the robot-assumed trust-behavior model $\hat{\pi}_b$, and the actual trust-behavior model $\tilde{\pi}_b$. \textcolor{black}{As we run the simulation 10,000 times, the maximum standard errors of $\overline{J}_m$ and $\overline{\hat{t}}_N$ in each bar are less than 1.5 and $1.3\times10^{-3}$ respectively.} }
  \label{fig:reward_trust_bar_comparison}
\end{figure*}



\subsection{Simulation Experiment 2: Comparing Team Performance and Trust}
In the second simulation experiment, we examine how different setups affect the team performance and the final trust. The team performance is defined as the total mission reward $J_m$ collected during the mission, as defined in Step 3) in Section~\ref{sec:procedure}. The final trust $\hat{t}_N$ is the expected value of trust after search all the $N$ sites and it is given by $\hat{t}_N=\frac{\alpha_N}{\alpha_N+\beta_N}$ due to Eq.~\eqref{eq:BetaTrust}.

To simulate the whole mission, we need the human's actual behavior model $\tilde{\pi}_b$ in addition to the two variables in the first experiment. $\tilde{\pi}_b$ has two levels, namely, ${\pi}_b^r$ and ${\pi}_b^d$. Besides the behavior models and the reward function, we also consider some other parameters' effect on the team performance. We tested different values of $\kappa_1,\kappa_2$ as a change of the relative threat detection accuracy of the robot. We also tested different values of $\alpha_1$ and $\beta_1$ to simulate different initial trust levels. Under each condition, we run the simulation 10,000 times over randomized $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ and calculate the mean value $\overline{J}_m$ of $J_m$ and the mean value $\overline{\hat{t}}_N$ of ${\hat{t}}_N$.

\textbf{Simulation result.} The simulation results are shown in Figure~\ref{fig:reward_trust_bar_comparison} and Table~\ref{tab:result2}. Figure~\ref{fig:reward_trust_bar_comparison} is the grouped bar-plot of $\overline{J}_m$ and $\overline{\hat{t}}_N$ under different settings. In the 2 groups on the left, $\alpha_1=100$ and $\beta_1=50$, so the initial trust is set to 0.67; while in the 2 groups on the right, the initial trust is 0.33. \textcolor{black}{Table~\ref{tab:result2} shows the mean and standard deviation of the team performance $J_m$ and final trust ${\hat{t}}_N$ correspondingly.} % \textcolor{blue}{\textbf{Observation 1: Asymmetry in the human's and robot's detection accuracy.} In  Figure~\ref{fig:reward_trust_bar_comparison}, a comparison between group 1 and 2 or group 3 and 4 shows that interchanging the values of $\kappa_1$ and $\kappa_2$ will result in different team performances. Additionally, when the robot starts trustworthy (group 1 and 2) and has the higher detection accuracy then the team has a better performance. This is a consequence of that the robot has a long planning horizon so the team will benefit from giving the robot the better detection accuracy. }

\textbf{Observation 1: High-ability trustworthy robot results in high team performance and high trust.} In Figure~\ref{fig:reward_trust_bar_comparison}, a comparison between the first 2 groups, where the initial trust is relatively high, shows that if we increase the robot's threat-detection accuracy by changing $\kappa_2$ from 2 to 50, no matter which setup the model uses, both the team performance and the final trust increase. \textcolor{black}{However, in the last two groups, where the initial trust is low, the team performance does not always increase with the robot's ability. Particularly, when the robot-assumed trust-behavior model is correct ($\hat{\pi}_b=\tilde{\pi}_b$), the team performance increases when the robot's detection accuracy is higher; while when the robot-assumed trust-behavior model is wrong ($\hat{\pi}_b \neq \tilde{\pi}_b$), the team performance may not increase with the robot's detection accuracy. This can be explained by the fact that the two trust-behavior models differ mostly in the low-trust situation, so the robot may make a sub-optimal decision when its assumed trust-behavior model is wrong and the human's trust is low.}
% robot's threat-detection accuracy by changing $\kappa_2$ from 2 to 50, no matter which setup the model uses, both the team performance and the final trust increase.

\textbf{Observation 2: Trust-seeking reward does not harm team performance when the robot is trustworthy.} \textcolor{black}{Within each group, the $i+4$th bar uses the same condition as the $i$th one's except that their reward functions are different, $i=1,2,3,4$.} In the first 2 groups, where the initial trust is set to 0.67, when changing reward from $R_m$ to $R_t$, team performance \textcolor{black}{barely decreases} while the final trust increases; however, in the last 2 groups, where the initial trust is 0.33, \textcolor{black}{the team performance decreases in some cases}, which can be thought of as a compensation for the increment in the trust. Therefore, if the robot starts in a high-trust state, then seeking trust will not harm the long-term team performance, while if it starts in a low-trust state, insisting to gain trust will cause the team performance to decrease.

\textbf{Observation 3: Low initial trust does not lead to low team performance in the reverse psychology model.} In the first bar in each group, both the robot's assumed trust-behavior model $\hat{\pi}_b$ and the human's actual behavior $\tilde{\pi}_b$ are the reverse psychology model ${\pi}^r_b$. Comparing the first bars in the 1st group and the 3rd group shows that the team performance increases when the initial trust decreases from $(\alpha_1{=}100,\beta_1{=}50)$ to $(\alpha_1{=}50,\beta_1{=}100)$. This can be explained by the fact that, in the POMDP, both low-trust states and high-trust states have high values (expected team performance), however, a perceived failure has a larger impact on trust than a perceived success, and thus manipulating the human to a low-trust condition will let the robot reach a high-value state faster.


\textbf{Observation 4: a disuse-human performs better than a reverse-psychology human when working with a trustworthy robot.} Within each of the first 2 groups, where the robot is trustworthy (initial trust level is 0.67), the team performance is higher when the actual trust-behavior model is the disuse model ($\tilde{\pi}_b=\pi_b^d$, bar 2, 4, 6, and 8) than the team performance of the reverse psychology model ($\tilde{\pi}_b=\pi_b^r$, bar 1, 3, 5, and 7). This observation indicates that the team can achieve high performance as long as the human uses the disuse strategy no matter what the robot-assumed trust-behavior is, even when the robot-assumed model doesn't match the actual model. However, this is not true in the last two groups, wherein the initial trust is low (0.33). 
% when the human doesn't trust the robot. The second bar in group 3 indicates the team performance is low when a low-ability human ($\kappa_1=2$) disuses a high-ability robot ($\kappa_2=50$).

% \textbf{Observation 5: a Nash equilibrium point in the trust-driven HRI.} If we view the choices of trust-behavior models as a two-player game between the robot and the human to maximize team performance, in a sense that the human chooses his or her actual trust-behavior model and the robot chooses its assumed trust-behavior model, then both of them choosing the disuse model is the Nash equilibrium of this game. Indeed, within each group in Figure~\ref{fig:reward_trust_bar_comparison}, the team performance and the final trust are the highest when both of them choose the disuse model (bar 4, bar 8), and thus any of them moving from this point would result in lower team performance. This observation indicates that, regardless of the initial trust and the robot's ability, both the robot and the human should assume disuse trust-behavior to maximize team performance.    

\section{Conclusion}\label{sec:discussion}
Our study is the first attempt to examine the trust-behavior models in detail.  We proposed two trust-behavior models and investigated how the different models affect a robot's optimal policy and HRI team performance. Results indicate that if the robot assumes that the human uses the reverse psychology model, it will deliberately `manipulate' the human when the human's trust is low. The reward function with the added trust seeking term can potentially prevent this \textcolor{black}{``manipulative''} behavior. \textcolor{black}{Our study should be viewed in light of the following limitations. First, the concept of trust has been examined in various disciplines including human-robot interaction \cite{Sheridan:2016kn}, organizational management \cite{Mayer:1995ju}, psychology \cite{Klimoski1976}, and social philosophy \cite{Faulkner2017}. The diverse interest has generated multiple definitions of trust. In our study, we use one of the widely used definitions in human-autonomy interaction. Further research should consider alternative definitions from other disciplines. Please see \cite{Lewis2018,Mayer:1995ju} for more discussion on the definitions of trust. Second, the trust dynamics model used in the present study is primarily ability-centric. Even though the focus of the present study is not on the trust dynamics model, further research should be conducted to validate the simulation findings when a more inclusive trust dynamics model is available. Such dynamics models could consider additional characteristics of the trustee including the trustee's benevolence and integrity.}
% In addition, our results revealed that under certain scenarios, a Nash equilibrium occurs if both the robot and the human assume the disuse trust-behavior model to achieve maximum team performance. 
% The observations in the results are under our proposed scenario. Further research directions can be to release the assumptions and generalize the observations.







==> RA-L_ICRA 2021 HRI simulation/big_whole_page_figure.tex <==
\begin{figure*}[h]
  \centering
    \begin{subfigure}{1\textwidth}
    \captionsetup{width=1.1\linewidth}
  \centering
        \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_11_rev_mission.pdf}
        \caption{Reverse-psychology-based trust-behavior model ($\hat{\pi}_b = {\pi}_b^r$) and mission reward ($R=R_m$).}
        \label{fig:a}
    \end{subfigure}
    \begin{subfigure}{1\textwidth}
    \captionsetup{width=1.1\linewidth}
    \vspace{3mm}
  \centering
  \vspace{5pt}
        \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_12_rev_trust.pdf}
        \caption{Reverse-psychology-based trust-behavior model ($\hat{\pi}_b = {\pi}_b^r$) and trust-seeking reward ($R=R_t$).}
        \label{fig:b}
    \end{subfigure}  
    \begin{subfigure}{1\textwidth}
    \captionsetup{width=1.1\linewidth}
    \vspace{3mm}
  \centering
  \vspace{5pt}
        \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_21_dis_mission.pdf}
        \caption{Disuse-based trust-behavior model ($\hat{\pi}_b = {\pi}_b^d$) and mission reward ($R=R_m$).}
        \label{fig:c}
    \end{subfigure}  
    \begin{subfigure}{1\textwidth}
    \captionsetup{width=1.1\linewidth}
    \vspace{2mm}
  \centering
  \vspace{5pt}
        \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_22_dis_trust.pdf}
        \caption{Disuse-based trust-behavior model ($\hat{\pi}_b = {\pi}_b^d$) and trust-seeking reward ($R=R_t$).}
        \label{fig:d}
    \end{subfigure}  
    % \hspace{0.2cm}
    \caption{Action functions and value functions of the POMDP model under different settings. In each sub-figure, the top row are the images of the action functions of different sites. The horizontal axis stands for $\alpha_k$ and the vertical axis stands for $\beta_k$. \textcolor{black}{For a fixed $\alpha_k$, larger $\beta_k$ means lower trust; while, for a fixed $\beta_k$, larger $\alpha_k$ means higher trust.} Black area are the states whose optimal action $A_k(\alpha_k,\beta_k)$ is zero, i.e., the robot should not recommend the human to wear the protective gear, and vice versa. In each sub-figure, the bottom row are the images of the value functions of different sites. The brighter a state $(\alpha_k,\beta_k)$ is, the higher its value $V_k(\alpha_k,\beta_k)$ is. For a better visualization, we use different colormaps for different value functions. So values cannot be compared across different images by the color.}
  \label{fig:V_A_functions}
\end{figure*}



==> RA-L_ICRA 2021 HRI simulation/table-experiment2Result.tex <==
\begin{table*}[!h]
\caption{Team performance and final trust under different setups in experiment 2}
\caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
\label{tab:result2}
\centering
% \tabcolsep=0.05cm
\scalebox{0.99}{
\begin{tabular}{c|c|c|c|c|cc}
\hline
\multirow{2}{*}{$R$}   & \multirow{2}{*}{$\hat{\pi}_b$} & \multirow{2}{*}{$\tilde{\pi}_b$} & \multicolumn{2}{c|}{$\alpha_1=100$,   $\beta_1=50$}      & \multicolumn{2}{c}{$\alpha_1=50$,   $\beta_1=100$}                            \\ \cline{4-7} 
                       &                                &                                  & $\kappa_1=2$, $\kappa_2=2$ & $\kappa_1=2$, $\kappa_2=50$ & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=2$} & $\kappa_1=2$, $\kappa_2=50$ \\ \hline
\multirow{4}{*}{$R_m$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -816(±145), 0.55(±0.13)    & -798(±144), 0.60(±0.13)     & \multicolumn{1}{c|}{-791(±142), 0.24(±0.06)}    & -768(±144), 0.22(±0.05)     \\ \cline{3-7} 
                       &                                & $\pi_b^d$                        & -744(±149), 0.55(±0.13)    & -716(±150), 0.60(±0.13)     & \multicolumn{1}{c|}{-803(±144), 0.24(±0.06)}    & -809(±142), 0.22(±0.05)     \\ \cline{2-7} 
                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -819(±144), 0.59(±0.08)    & -801(±147), 0.63(±0.08)     & \multicolumn{1}{c|}{-876(±144), 0.45(±0.08)}    & -878(±143), 0.48(±0.07)     \\ \cline{3-7} 
                       &                                & $\pi_b^d$                        & -723(±138), 0.59(±0.08)    & -700(±136), 0.63(±0.08)     & \multicolumn{1}{c|}{-727(±138), 0.45(±0.08)}    & -711(±137), 0.48(±0.07)     \\ \hline
\multirow{4}{*}{$R_t$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -818(±145), 0.59(±0.08)    & -801(±144), 0.63(±0.08)     & \multicolumn{1}{c|}{-842(±140), 0.35(±0.10)}    & -833(±137), 0.35(±0.12)     \\ \cline{3-7} 
                       &                                & $\pi_b^d$                        & -725(±139), 0.59(±0.08)    & -698(±138), 0.63(±0.08)     & \multicolumn{1}{c|}{-762(±146), 0.35(±0.11)}    & -763(±152), 0.35(±0.12)     \\ \cline{2-7} 
                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -820(±146), 0.59(±0.08)    & -800(±145), 0.63(±0.08)     & \multicolumn{1}{c|}{-874(±141), 0.45(±0.08)}    & -877(±142), 0.48(±0.07)     \\ \cline{3-7} 
                       &                                & $\pi_b^d$                        & -725(±139), 0.59(±0.08)    & -700(±136), 0.63(±0.08)     & \multicolumn{1}{c|}{-730(±138), 0.45(±0.07)}    & -713(±137), 0.48(±0.07)     \\ \hline
\end{tabular}
}
\vspace{-4mm}
\end{table*}


==> RA-L_ICRA 2021 HRI simulation/table-experiment2Result_backup.tex <==
\begin{table*}[!h]
\caption{Team performance and final trust under different setups in experiment 2}
\caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
\label{tab:result2}
\centering
\tabcolsep=0.05cm
\scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|ccc}
\hline
\multirow{2}{*}{$R$}   & \multirow{2}{*}{$\hat{\pi}_b$} & \multirow{2}{*}{$\tilde{\pi}_b$} & \multicolumn{3}{c|}{$\alpha_1=100$,   $\beta_1=50$}                                    & \multicolumn{3}{c}{$\alpha_1=50$,   $\beta_1=100$}                                                                               \\ \cline{4-9} 
                       &                                &                                  & $\kappa_1=2$, $\kappa_2=2$ & $\kappa_1=2$, $\kappa_2=50$ & $\kappa_1=50$, $\kappa_2=2$ & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=2$} & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=50$} & $\kappa_1=50$, $\kappa_2=2$ \\ \hline
\multirow{4}{*}{$R_m$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -816(±145), 0.55(±0.13)    & -798(±144), 0.60(±0.13)     & -816(±143), 0.55(±0.13)     & \multicolumn{1}{c|}{-791(±142), 0.24(±0.06)}    & \multicolumn{1}{c|}{-768(±144), 0.22(±0.05)}     & -790(±144), 0.24(±0.06)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -744(±149), 0.55(±0.13)    & -716(±150), 0.60(±0.13)     & -743(±149), 0.56(±0.13)     & \multicolumn{1}{c|}{-803(±144), 0.24(±0.06)}    & \multicolumn{1}{c|}{-809(±142), 0.22(±0.05)}     & -803(±142), 0.24(±0.06)     \\ \cline{2-9} 
                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -819(±144), 0.59(±0.08)    & -801(±147), 0.63(±0.08)     & -819(±144), 0.59(±0.08)     & \multicolumn{1}{c|}{-876(±144), 0.45(±0.08)}    & \multicolumn{1}{c|}{-878(±143), 0.48(±0.07)}     & -877(±144), 0.45(±0.07)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -723(±138), 0.59(±0.08)    & -700(±136), 0.63(±0.08)     & -726(±138), 0.59(±0.08)     & \multicolumn{1}{c|}{-727(±138), 0.45(±0.08)}    & \multicolumn{1}{c|}{-711(±137), 0.48(±0.07)}     & -728(±139), 0.45(±0.07)     \\ \hline
\multirow{4}{*}{$R_t$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -818(±145), 0.59(±0.08)    & -801(±144), 0.63(±0.08)     & -818(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-842(±140), 0.35(±0.10)}    & \multicolumn{1}{c|}{-833(±137), 0.35(±0.12)}     & -856(±140), 0.39(±0.10)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -725(±139), 0.59(±0.08)    & -698(±138), 0.63(±0.08)     & -722(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-762(±146), 0.35(±0.11)}    & \multicolumn{1}{c|}{-763(±152), 0.35(±0.12)}     & -749(±149), 0.39(±0.10)     \\ \cline{2-9} 
                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -820(±146), 0.59(±0.08)    & -800(±145), 0.63(±0.08)     & -817(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-874(±141), 0.45(±0.08)}    & \multicolumn{1}{c|}{-877(±142), 0.48(±0.07)}     & -878(±144), 0.45(±0.07)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -725(±139), 0.59(±0.08)    & -700(±136), 0.63(±0.08)     & -723(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-730(±138), 0.45(±0.07)}    & \multicolumn{1}{c|}{-713(±137), 0.48(±0.07)}     & -725(±139), 0.45(±0.07)     \\ \hline
\end{tabular}
}
\end{table*}


==> RA-L_ICRA 2021 HRI simulation/table-experiment2Result_backup2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% old table %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}
% \caption{Team performance and final trust under different setups}
% \caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
% \label{tab:result2}
% \centering
% \begin{tabular}{c|c|c|c|c|cc}
% \hline
% \multirow{2}{*}{$R$}   & \multirow{2}{*}{$\hat{\pi}_b$} & \multirow{2}{*}{$\tilde{\pi}_b$} & \multicolumn{2}{c|}{$\alpha_1=100$,   $\beta_1=50$}       & \multicolumn{2}{c}{$\alpha_1=50$,   $\beta_1=100$}                             \\ \cline{4-7} 
%                       &                                &                                  & $\kappa_1=2$, $\kappa_2=50$ & $\kappa_1=50$, $\kappa_2=2$ & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=50$} & $\kappa_1=50$, $\kappa_2=2$ \\ \hline
% \multirow{4}{*}{$R_m$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -798(±144), 0.60(±0.13)     & -816(±143), 0.55(±0.13)     & \multicolumn{1}{c|}{-768(±144), 0.22(±0.05)}     & -790(±144), 0.24(±0.06)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -716(±150), 0.60(±0.13)     & -743(±149), 0.56(±0.13)     & \multicolumn{1}{c|}{-809(±142), 0.22(±0.05)}     & -803(±142), 0.24(±0.06)     \\ \cline{2-7} 
%                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -801(±147), 0.63(±0.08)     & -819(±144), 0.59(±0.08)     & \multicolumn{1}{c|}{-878(±143), 0.48(±0.07)}     & -877(±144), 0.45(±0.07)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -700(±136), 0.63(±0.08)     & -726(±138), 0.59(±0.08)     & \multicolumn{1}{c|}{-711(±137), 0.48(±0.07)}     & -728(±139), 0.45(±0.07)     \\ \hline
% \multirow{4}{*}{$R_t$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -801(±144), 0.63(±0.08)     & -818(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-833(±137), 0.35(±0.12)}     & -856(±140), 0.39(±0.10)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -698(±138), 0.63(±0.08)     & -722(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-763(±152), 0.35(±0.12)}     & -749(±149), 0.39(±0.10)     \\ \cline{2-7} 
%                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -800(±145), 0.63(±0.08)     & -817(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-877(±142), 0.48(±0.07)}     & -878(±144), 0.45(±0.07)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -700(±136), 0.63(±0.08)     & -723(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-713(±137), 0.48(±0.07)}     & -725(±139), 0.45(±0.07)     \\ \hline
% \end{tabular}
% \end{table*}

==> RA-L_ICRA 2021 HRI simulation/z_commented_text_backup.tex <==

% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve how people live and work; however, their sophisticated underlying algorithms make themselves uncertain and inexplicable. Consequently, people need to establish appropriate trust in them to to fully realize the potential of these technologies. 



% We simulated and compared both models' effects on trust-aware decision making and found that the robot will ``manipulate'' the human's trust if it assumes the human uses reverse psychology. To overcome this ``unethical'' behavior, we proposed a trust-seeking reward function to  


% \textbf{We make the following contributions in this study:}
% \begin{itemize}
%     \item We proposed and compared different trust-behavior models to show how disuse and reverse psychology would affect trust-aware decision making and the human-robot team's performance. 
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}

% , , a robot should be able to estimate a human's trust accurately in real time, anticipate how trust influences the subsequent interactions, and consequently choose the optimal action that maximizes a given goal. These three steps correspond to three major components in trust-aware HRI, i.e., trust dynamics, trust-behavior model, and trust-aware decision-making framework. 

% Two major components in a trust-aware HRI model are the trust dynamics model and the trust-behavior model.

% In addition, some unique properties of robots result in more factors influencing trust, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}.

% Traditional research on human-automation highlights the strong connection between trust and automation's reliability. Lee and Moray~\cite{Lee:1992it} identified the three dimensions of trust in automation as \textit{performance}, \textit{process}, and \textit{purpose}, where performance is the automation's reliability to achieve the operator’s goals, process is the degree to which the automation’s algorithms are appropriate for the situation and the operator’s goals, and purpose refers to the degree to which the automation is being used within the realm of the designer’s intent. Because automation lacks intentionality~\cite{lee2004trust} and is often designed to fulfill the operator's goals, trust in automation is largely determined by its first dimension, namely, its performance. As a result, a majority of related research focuses on how to calibrate human trust based on the performance of the automation. However, when it comes to a complex system, e.g., a humanoid robot assistant, it is difficult for the users to tell how reliable the system is. Additionally, when a robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust. Therefore, recently, researchers proposed trust-aware human-robot interaction (HRI) models to examine how trust affects a robot's reasoning and task performance~\cite{chen2020trust}. 

% Two major components in a trust-aware HRI model are the trust dynamics model and the trust-behavior model. A trust dynamics model specifies how human trust changes in response to the robot's action and environmental change and a trust-behavior model describes what the human will do at different trust levels. Numerous research has investigated trust dynamics, however, few has investigated trust behavior in HRI. In this study, we proposed two different ways to model trust behavior, i.e., the disuse model and the reverse psychology model. In the disuse model, a human will completely ignore the robot and use his own policy when trust is below a certain level; while in the reverse psychology model, the human will do the opposite to what the robot tells him when his trust is low. We compared their effects on trust-aware decision making and found that the robot will manipulate the human's trust if it assumes the human uses reverse psychology. To overcome this ``unethical'' behavior, we proposed a trust-seeking reward function to  

% \textbf{Generally, we make the following contributions in this study:}
% \begin{itemize}
%     \item We compared different trust-behavior model to show how disuse and reverse psychology would affect a trust-aware robot's decision and the human-robot team's performance.
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}

% The paper is organized as follows: Sec.~\ref{sec:relatedWork} reviews related work in trust-driven human-robot interaction; Sec.~\ref{sec:model} formulate the problem in a POMDP framework and proposed the reverse psychology trust-behavior model as well as the trust-seeking reward function; in Sec.~\ref{sec:case}, we introduced a reconnaissance mission as a study case to examine how different settings affect the interaction; Sec.~\ref{sec:result} reports the simulation results and our observations; in Sec.~\ref{sec:discussion} we summarized our findings and discussed the limitations and future directions of this study. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% previous introduction               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Developments in technology enable robots to help human in a variety of fields. However, sophisticated robotic systems make themselves complex and uncertain, and thus a human agent need to establish an appropriate level of trust in a robot to enable efficient human-robot. Trust is defined as ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"

% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve every sector of our economy and improve how people live and work. It is predicted that the number of robots in use worldwide will multiply even faster in the next 10 years, reaching as many as 20 million by 2030 \cite{OxfordEconomics2019}. However, realizing the full economic, safety and health potential of these technologies is only possible if people establish appropriate trust in them. 


% Since any robot is essentially an automated machine, human-robot trust exhibits most properties of human-automation trust. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% Since any robot is essentially an automated machine, trust in robots and trust in automation have a close relation. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust the automation so they use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% To illustrate these two points, let's consider a reconnaissance mission as an example, which will be used through out our study. Suppose a soldier teams up with a robot to search several sites in a town for terrorists. The robot enters each site initially, scanning for potential threats and then recommends to the soldier if he should wear protective gear before entering the site. The protective gear is heavy and wearing it is time-consuming. If the soldier with the protective gear enters a site and finds no threat, the human-robot team wastes precious time; conversely, if the solider decides not to wear the protective gear, he will harmed if threat is present. The goal of the human-robot team is to minimize the soldier's health loss while to complete the mission as soon as possible, which can be possibly realized as minimizing the sum of the mission time and the soldier's health decrements. We should note the sub-goals conflict with each other and, as a consequence, the robot may deliberately manipulate the soldier if trust is considered in its reasoning. For instance, suppose the mission is under high time pressure, if the robot senses that the soldier's trust is high, it may not recommend the soldier to wear the protective gear no matter what the scanned result is; on the contrary, if the robot knows the soldier has a low trust in it, it may suggest the soldier to wear the protective gear based on the `reverse psychology'~\cite{macdonald2011people}. 

% This example demonstrates that, first, although in the reconnaissance mission the soldier may construe the reliability of the robot as its detection accuracy, the recommendation given by the robot actually serves for the goal to minimize the sum of the mission duration and soldier's health loss and thus is not necessarily based on the presence of the threat. As a result, the soldier may not clearly understand what the reliability of the robot is. Second, the robot chooses different actions on different trust level, which indicates the \textit{perceived reliability} of the robot depends on the soldier's trust.


% These two points shows that there is a substantial difference between human-automation trust and human-robot trust. Traditional research on human-robot trust follows the pattern of human-automation trust research on trust calibration, with an emphasis on how trust will be affected by some unique properties of robots, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}. Recently, researchers began to embed human trust in a robot's reasoning process, showing that maximizing trust does not mean maximizing the objective of a human-robot team~\cite{chen2020trust} and it is possible the robot will manipulate human's trust even the designer does not intent to do so~\cite{losey2019robots}. These studies raised the concern that only calibrating human-robot trust to a constant 'appropriate' level may not be enough for best system performance and there may be unseen problem, such as taking advantage of human's trust, when designing a robot's algorithm. Inspired by these concerns, in this study, we analyzed how different trust-behavior model would affect a robot's trust-aware planning and proposed a method to keep the robot from manipulating human trust.


% \textit{misuse} and \textit{disuse} are two major concepts used in research on trust in automation, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% \textcolor{red}{Jessie: @Yaohui, the difference between human-automation and human-robot interaction is too strong an assumption. People will have difficulty buying in. I suggest: 1. do not try to make the distinction between the two types of trust. 2. move the scenario to a later section, perhaps section 3. 3. move the trust updating assumption to a later section, perhaps create another sub-section in section 3 to briefly describe the trust updating model and state that in this paper we will also use this more with the assumption.}

% As any robot is essentially an automated machine, human-robot trust is a descendant of human-automation trust. In the past three decades Researchers has extensively studied trust in automation and generated different definition of it. Lee and See~\cite{lee2004trust} summarized related work and define trust in automation as  

% Trust in automation, or more recently trust in autonomy, has received extensive research interest and has been defined as a belief, an attitude, and a behavior \cite{Lewis2018}. In this paper, we use the definition by Lee and See~\cite{See:2004vj}: Trust is the ``attitude that an (autonomous) agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (see ~\cite{Lewis2018} for discussions on the definitions of trust). \textit{We make a clear distinction between trust and trusting behaviors.} Trust is an individual's attitude internal to him- or her-self. Trusting behaviors are behaviors displayed by the individual that can be observed and measured directly. 

% Two major concepts in human-automation trust research are \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% [Mention Conflicting studies on trust behavior]
% \textbf{Generally, we make the following contributions in this study:}
% \begin{itemize}
%     \item We compared different trust-behavior model to show how disuse and reverse psychology would affect a trust-aware robot's decision. [To add more detail]
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}


% Trust has been defined as a belief, an attitude, or a behavior \cite{Lewis2018} in different contexts. In this study, we use a general definition given by Lee and See~\cite{See:2004vj} which can fit into most scenarios:  trust is the ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability".




% Trust in automation, or more recently trust in autonomy, has received extensive research interest and has been defined as a belief, an attitude, and a behavior \cite{Lewis2018}. In this paper, we use the definition by Lee and See~\cite{See:2004vj}: Trust is the ``attitude that an (autonomous) agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (see ~\cite{Lewis2018} for discussions on the definitions of trust). \textit{We make a clear distinction between trust and trusting behaviors.} Trust is an individual's attitude internal to him- or her-self. Trusting behaviors are behaviors displayed by the individual that can be observed and measured directly. 


% [transition] We will use the definition of trust given by Lee and See~\cite{lee2004trust}: \textit{"attitude that an agent will help achieve an individual’s goals in a situation characterized by uncertainty and vulnerability."}
% past three decades~\cite{hoff2015trust, lee2004trust}.
% Compared with traditional research in human-robot trust, which mainly focuses on identifying factors that influence human trust as well as how to calibrate human trust based on the automation's reliability, recent research in human-robot trust trends to explicitly model human trust into a robot's reasoning process to help it better collaborate with a human agent~\cite{kok2020trust}. In the latter case, the model usually compose the robot will treat human trust as a state variable and keep updating a belief over the human agent's trust and choose if the robot and the human agent do not share the same goal, the robot
% definition of trust~\cite{lee2004trust}

% Since a robot is essentially an automated machine, dynamics of human-robot trust inherits most of its properties from human-automation trust. 

% More than two dozen factors have been identified to influence trust in automation, including individual factors such as culture and age~\cite{Rau2009, McBride:2011ix}, system factors such as reliability~\cite{Salem2015, Wickens:2009False}, and environmental factors such as multi-tasking requirement and task emergency~\cite{Robinette:2016_HRI, Zhang2017:HFES} (See~\cite{Hoff:2015fuba, Schaefer:2016hp} for a full list of factors). In addition, some unique properties of robots result in more factors influencing trust, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}.

% Researchers also examined trust adjustment based on interaction with automation. Manzey et al.~\cite{Manzey:2012hm} noted two feedback loops in the human agent's trust adjustment process, namely a positive loop triggered by automation success and a negative loop triggered by automation failure. The negative feedback loop exerts a stronger influence on trust adjustment than the positive feedback loop. Moreover, Desai et al.~\cite{Desai:2013cmbaca} found that the timing of automation failures, namely, at the beginning, middle, or end of an human-robot interaction task also affected how human operators adjusted their trust: A stronger drop of trust was observed when the automation failures occurred near the end than at the start or in the middle. Yang et al.~\cite{Yang:2017:EEU:2909824.3020230} examined how trust in automation evolved as an \textit{average human agent} gained experience interacting with robotic agents. Their study showed that the average human agent's trust in automation stabilized over repeated interactions, and this process can be modeled using a first-order linear time-invariant dynamic system.



% These two points shows that there is a substantial difference between human-automation trust and human-robot trust. Traditional research on human-robot trust follows the pattern of human-automation trust research on trust calibration, with an emphasis on how trust will be affected by some unique properties of robots, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}. Recently, researchers began to embed human trust in a robot's reasoning process, showing that maximizing trust does not mean maximizing the objective of a human-robot team~\cite{chen2020trust} and it is possible the robot will manipulate human's trust even the designer does not intent to do so~\cite{losey2019robots}. These studies raised the concern that only calibrating human-robot trust to a constant 'appropriate' level may not be enough for best system performance and there may be unseen problem, such as taking advantage of human's trust, when designing a robot's algorithm. Inspired by these concerns, in this study, we analyzed how different trust-behavior model would affect a robot's trust-aware planning and proposed a method to keep the robot from manipulating human trust.


% Trust in autonomy is a person's ``attitude that an (autonomous) agent will help achieve an individual's (his or her) goals in a situation characterized by uncertainty and vulnerability \cite{See:2004vj}." 
% To investigate trust in autonomy, the majority of studies have used a ``snapshot" view and evaluated trust with questionnaires administered at the end of an experiment. More than two dozen factors have been identified to influence the (snapshot) trust in autonomy. These factors can be broadly categorized into individual factors such as culture and age \cite{Rau2009, McBride:2011ix}, system factors such as reliability \cite{Salem2015, Wickens:2009False}, and environmental factors such as multi-tasking requirement and task emergency \cite{Robinette:2016_HRI, Zhang2017:HFES} (See \cite{Hoff:2015fuba, Schaefer:2016hp} for a full list of factors). However, this ``snapshot" view does not acknowledge that trust is a dynamic variable that can strengthen and decay over time.  With few exceptions (e.g., \cite{Lee:1992it, Manzey:2012hm, Guo2020_IJSR, Desai:2013cmbaca, Yang:2017:EEU:2909824.3020230}), we have little understanding of the temporal dynamics of trust formation and evolution, nor of how trust strengthens or decays over time as a result of moment-to-moment interactions in human-autonomy teams \cite{Yang:2017:EEU:2909824.3020230, DeVisser2020}. 

% To examine trust adjustment based on moment-to-moment interaction with autonomy, Manzey et al.  \cite{Manzey:2012hm} noted two feedback loops in the human agent's trust adjustment process, namely a positive and a negative feedback loop. The positive loop is triggered by experiencing automation success, and the negative loop by experiencing automation failure. The negative feedback loop exerts a stronger influence on trust adjustment than the positive feedback loop. Moreover, Desai et al. \cite{Desai:2013cmbaca} found that the timing of automation failures, namely, at the beginning, middle, or end of an human-robot interaction task also affected how human operators adjusted their trust: A stronger drop of trust was observed when the automation failures occurred near the end than at the start or in the middle. Yang et al. \cite{yang2016} observed the hindsight bias when human agents' adjust their trust in autonomy, that an autonomy failure was forgiven to some extent if the failure did not harm the team performance. 
% In the second category, researchers are focused on building a mathematical function for describing or predicting trust dynamics.
% Besides the empirical studies, In addition, Lee and Moray~\cite{Lee:1992it} proposed an auto-regressive moving average vector (ARMAV) time series model of trust which calculated trust at the present moment $t$ as a function of trust at the previous moment $t-1$, task performance, and the occurrence of automation failures. Yang et al.~\cite{Yang:2017:EEU:2909824.3020230} examined how trust in automation evolved as an \textit{average human agent} gained experience interacting with robotic agents. Results of their study showed that the average human agent's trust in automation stabilized over repeated interactions, and this process can be modeled using a first-order linear time-invariant dynamic system. The above-mentioned studies provide valuable insight into the trust dynamics of an average human agent. More recent studies used a data-driven approach to model trust dynamics. In this approach, trust is considered as information internal to the human that is not directly observable but can be inferred from other observable information \cite{Xu:2015cc}. For example, Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's electroencephalography (EEG) and galvanic skin response (GSR) data. Similarly, Lu and Sarter~\cite{lu2019eye} proposed the use of eye-tracking metrics including fixation duration and scan path length to infer the human's real-time trust. Their follow-up study \cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level. Instead of using physiological signals, Xu and Dudek~\cite{xu2015optimo} built an online probabilistic trust inference model based on the dynamic Bayesian network framework, treating the human agent's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human agent's behavior. In \cite{xu2015optimo} the trust dynamics of each individual human agent was modeled. 


% The above mentioned data-driven methods provided insights on how to predict a human's real-time trust by analyzing other observable information. However, they were subject to two limitations. First, some of them depend on using physiological sensors such as EEG and eye-tracking devices, which could be intrusive or be sensitive to noises \cite{hu2016real,Lu2019,Lu2020}. Second, as none of the existing models fully considered the empirical results showing how human agents adjust their trust \textit{de facto}, the resulting models could be limited in model explicability and generalizability. 

% Since robots belong to the general automation, human-robot trust dynamics inherits many properties from human-automation trust. Lee and See summ

% Review~\cite{hancock2011meta}

% Lu and Sarter~\cite{lu2019eye} showed that people visit more frequently and spend more time on low reliable automation.

% Wang et al.~\cite{wang2016trust} showed that adding explanation capability to a robot led to improvement in transparency, trust, and team performance in HRI.

% \subsection{Computational Trust Modeling}

% Trust should be numerically represented to fit in algorithms.

% Xu and Dudek~\cite{xu2015optimo} proposed the OPTIMo, which stands for the online probabilistic trust inference model, to estimate a human agent's real-time trust based on the automation's performance and the human agent's behavior.

% Hu et al.~\cite{hu2016real} proposed to estimate trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's psychophysiological measurements, i.e., electroencephalography (EEG) and galvanic skin response (GSR) data.

% Lu ~\cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level.

% Guo \cite{guo2020modeling}

% game theory

% Because the majority of research in human-automation research focuses on calibrating trust to an appropriate level, few studies considered how human behaves when trust diverges from this level. 


% Further more, research shows a certain low trust level may not result in a unique trust behavior. For example, Robinette~\cite{robinette2016overtrust} showed, in a simulated emergency evacuation scenario, the participants exhibited overtrust behavior to follow a guiding robot even though they did not trust the robot. To resolve such conflicting relation, Lee and See~\cite{lee2004trust} proposed a framework shows that behaviors are results of intentions and that intentions are a function of attitudes. Because trust is only one of the factors in a human's attitude, it cannot completely determine intention and thus cannot determine behavior. To predict behavior, a model of other attitude factors is needed, such as workload, attention, and self-confidence of the human. As a result, trust-behavior models should be highly contextual. For instance, Chen et al.~\cite{chen2020trust} found that human behavior in HRI is determined by both trust and risk of the task. 


% While it is widely accepted that low trust level in automation will lead to disuse and high trust level will lead to reliance, there is few studies on how a human would behave if he is at a trust level and not willing to collaborate with a robot. Research shows a certain low trust level may not result in a unique trust behavior. For example, Robinette~\cite{robinette2016overtrust} showed, in a simulated emergency evacuation scenario, the participants exhibited overtrust behavior to follow a guiding robot even though they did not trust the robot. To resolve such conflicting relation, Lee and See~\cite{lee2004trust} proposed a framework shows that behaviors are results of intentions and that intentions are a function of attitudes. Because trust is only one of the factors in a human's attitude, it cannot completely determine intention and thus cannot determine behavior. To predict behavior, a model of other attitude factors is needed, such as workload, attention, and self-confidence of the human. As a result, trust-behavior models should be highly contextual.



%  often take the form of embedding the Theory of Mind (ToM) 
% in a partially observable Markov decision process~\cite{kok2020trust}. ToM enables a robot to keep a belief of a human's trust, and the 
% POMDP framework allows the robot to make decisions for maximizing its long-term performance. 



% We formulate the trust-aware HRI and propose two novel and viable trust-behavior models to characterize potential human behaviors when trust is low; and we propose a reward function that can prevent the robot from manipulating a human's trust while keep the task performance unharmed. 

% the reconnaissance mission in a partially observable Markov decision process (POMDP) framework and use the performance-induced trust model to model trust dynamics. The objective is to give soldiers `optimal' recommendations at each site $k$ during the reconnaissance mission, so as to maximized the overall rewards (including both time-to-completion and health related objectives). The `hidden' state is the trust level of soldier towards robot and needs to be constantly inferred in real-time during the mission. Vis-\`{a}-vis constructing the POMDP, we propose two novel and viable trust behaviors models depicting the soldier's response to the robot's recommendations.


% The true state is unobservable and it should be inferred through the observations. The robot runs the POMDP model during the interaction and solve for the optimal policy $\pi : B \rightarrow A$, which maps from the belief state space $B$ to action space, to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$

% We formulate the trust-aware HRI as a compact POMDP $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is the set of interaction states, $A$ is the set of robot's action, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $\Omega $ is the set of observations, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is the reward function specifying the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The true state is unobservable and it should be inferred through the observations. The robot runs the POMDP model during the interaction and solve for the optimal policy $\pi : B \rightarrow A$, which maps from the belief state space $B$ to action space, to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$



% POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi : B \rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$


% $g\in \{0,1\}$ indicates the soldier's decision of whether wearing the gear, where $g=1$ is to wear and $g=0$ is not to wear. $I$ encapsulates the information used in the soldier's decision making process. When the soldier has a higher trust $t$ in the robot, he will be more likely to follow the robot's recommendation. Denote the probability the soldier will follow the recommendation as $\varphi(\frac{\alpha }{\alpha +\beta })$, then $p( g=a\ |\ I)=\varphi (\frac{\alpha }{\alpha +\beta })$, which has been backed by Lee and See~\cite{lee2004trust}. To specify the soldier's behavior when he is \emph{not} following the recommendation, we consider two possible trust-behavior models, namely, the reverse psychology model and the disuse model, as shown in  Figure~\ref{fig:behaviors}. 


% \begin{equation}
% \pi_b^d(a_h,I) =\begin{cases}
% \varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \ \text{ following recommendation $g=a$},\\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)\tilde{d}_{k} & \ \text{ exercising self-judgement $g=1$}, \ \\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)( 1-\tilde{d}_{k}) & \ \text{ exercising self-judgement $g=0$}. 
% \end{cases}
% \end{equation}
% Contextually, given that the soldier does not follow the recommendation, we specify the probability of him wearing gear as $\tilde{d}_k$ and not wearing gear as $1-\tilde{d}_k$. 



% \begin{equation}
%   R_m(k)=\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right],
% \end{equation}
% At time $k$, the mission reward is given
% \begin{equation}
%   R_m(k)=\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right],
% \end{equation}



% \subsubsection*{\textbf{Trust-seeking reward to prevent manipulation.}} Later in the simulation study, we show if the robot only plans to maximize the mission reward $R_m$, it will deliberately \emph{manipulate} the soldier in the reverse psychology model. That is, the robot may deliberately make an opposite recommendation when the soldier's trust is low (so as to maximize potential reward). This is a result from the absence of trust in the mission reward $R_m$. However, purely maximizing human-trust would harm mission performance~\cite{chen2020trust}. So to correct this `unethical' behavior while let the robot focus on the mission goal, we propose a trust-seeking reward function
% \begin{equation}
% \label{trust-seeking}
%     R_t(k)=R_m(k) + \lambda(k)\mathds{1}(\mathcal{A}_k),
% \end{equation}
% where $\mathcal{A}_k$ is the event when the recommendation agrees with the ground truth, i.e., $r_k=\eta_k$, and $\lambda(k)$ is a positive weight and decreases when $k$ increases. The extra term $\lambda(k)\mathds{1}(\mathcal{A}_k)$ will force the robot to gain trust in near sites and optimize the mission reward in the long run.

% which can be possibly realized as minimizing the sum of the mission time and the soldier's health decrements.


% \frac{c}{1+e^{k}}
% \begin{table}[h]
% \caption{My Table}
% \vspace{-2mm}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Threat existence}                 \\ \cline{3-4} 
% \multicolumn{2}{|c|}{}                  & Yes                       & No                        \\ \hline
% \multirow{2}{*}{Protective gear}  & Yes & $(\delta_h ^{(1)},\delta_t^{(1)})$ & $(\delta_h^{(2)},\delta_t^{(2)})$ \\ \cline{2-4} 
%                                   & No  & $(\delta_h^{(3)},\delta_t^{(3)})$ & $(\delta_h^{(4)},\delta_t^{(4)})$ \\ \hline
% \end{tabular}
% \label{tab:weighted_sum}
% \end{table}\\
% And, for comparison, we will consider two trust behaviors to model how human react when his trust drops below a certain level, namely the disuse model and the reverse psychology model, and two objective function, namely the task objective and the task objective with added trust-seeking term. 
%  To put it in a POMDP framework, we model the robot's reasoning process as a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is the set of world states; $A={r,n}$ is the set of robot's action, where action $r$ means the robot recommends the soldier to wear the protective gear while action $n$ means the robot does not recommend to wear the gear; $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.
% \subsection{POMDP Framework}
% POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.\\
% In addition, we define the belief space $\displaystyle B:S\rightarrow [ 0,1]$ as the belief over all the states, and the reward function over the belief space as $\displaystyle \rho :B\times A\rightarrow \mathbb{R}$, which can be derived by $\displaystyle \rho ( b,a) =\sum\nolimits _{s\in S}\sum\nolimits _{s'\in S} R( s,a,s') T( s,a,s') b( s)$. The objective of a POMDP model is to find the optimal policy $\displaystyle \pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $\displaystyle J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.\\
% To estimate how much the human agent trusts the robot, we use the trust model proposed in [Trust reference paper]. We modeled trust by a Beta distribution whose parameters are updated according to the robot's performance.[Beta model here].\\
% when the human agent enters a building without protective gear, he will lose health $h_3$ and cost time $c_3$ when there are threats in the building, and lose health $h_4$ and cost time $c_4$ when there are no threats in the building. 

% We design two simulation experiments based on the reconnaissance mission described in Sec.~\ref{sec:case}, where we compare the robot's optimal policies and the human-robot team performance respectively under different trust-behavior models and reward functions.  


% \begin{table}[h]
% \caption{Parameter setting 1}
% \centering
% \begin{tabular}{cl|cl}
% \hline
% Parameter  & Value & Parameter            & Value                     \\ \hline
% $N$        & 15    & $w^s$                & 10                        \\
% $w_h$      & 1     & $w^f$                & 20                        \\
% $w_t$      & 0.2   & $\gamma$             & 0.9                       \\
% $\kappa_1$ & 3     & $\lambda(k)$         & $\frac{80}{1+e^{0.5k}}$ \\
% $\kappa_2$ & 50    & $\mathcal{A}_k$      & $\eta_k=a_{r,k}$                          \\ \hline
% \end{tabular}
% \label{tab:exp1Parameters}
% \end{table}\\





% i.e., the disuse model and the reverse psychology model, as well as a trust seeking reward function. 
% We simulated a reconnaissance mission to


% This trust seeking term decreases as the planning step increases so it can force the robot to go to the high-trust state during the initial phase of interaction and meanwhile maximize long-term team performance. However, if the initial trust is low, forcing the robot to gain trust may sacrifice team performance. 



% We formulated the problem in a general framework, however, 

% I÷

% We formulated the problem in a general framework, how-ever, we imposed several assumption on the simulated casestudy, e.g., the robot and the human have the same goal andthe weights in the reward function favors the soldier’s health.If  these  assumption  is  dramatically  changed  the  results  canbe different. An extreme case is that, if the mission goal ischanged  to  only  minimize  the  time  cost,  then  the  soldier’soptimal action is always not wearing the gear and thus s/hecan stop using the robot. In addition, to simplify the model,we  assumed  the  probability  of  the  human  following  the robot’s recommendation as a linear function of trust. Furtherresearch is needed to investigate this relationship



==> RA-L_ICRA 2021 HRI simulation/z_previous_draft_backup.tex <==
% \section{Introduction}\label{sec:intro}
% % Developments in technology enables robots to help human in a variety of fields. However, sophisticated systems make themselves complex, unstable, and uncertain~\cite{lee2004trust}, thus human agents usually cannot follow a structured routine to interact with a robot and should establish an appropriate level of trust in the robot. 
% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve every sector of our economy and improve how people live and work. It is predicted that the number of robots in use worldwide will multiply even faster
% in the next 10 years, reaching as many as 20 million by 2030 \cite{OxfordEconomics2019}. However, realizing the full economic, safety and health potential of these technologies is only possible if people establish appropriate trust in them. 

% \textcolor{red}{Jessie: @Yaohui, the difference between human-automation and human-robot interaction is too strong an assumption. People will have difficulty buying in. I suggest: 1. do not try to make the distinction between the two types of trust. 2. move the scenario to a later section, perhaps section 3. 3. move the trust updating assumption to a later section, perhaps create another sub-section in section 3 to briefly describe the trust updating model and state that in this paper we will also use this more with the assumption.}


% Since any robot is essentially an automated machine, human-robot trust exhibits most properties of human-automation trust. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% % Since any robot is essentially an automated machine, trust in robots and trust in automation have a close relation. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust the automation so they use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% To illustrate these two points, let's consider a reconnaissance mission as an example, which will be used through out our study. Suppose a soldier teams up with a robot to search several sites in a town for terrorists. The robot enters each site initially, scanning for potential threats and then recommends to the soldier if he should wear protective gear before entering the site. The protective gear is heavy and wearing it is time-consuming. If the soldier with the protective gear enters a site and finds no threat, the human-robot team wastes precious time; conversely, if the solider decides not to wear the protective gear, he will harmed if threat is present. The goal of the human-robot team is to minimize the soldier's health loss while to complete the mission as soon as possible, which can be possibly realized as minimizing the sum of the mission time and the soldier's health decrements. We should note the sub-goals conflict with each other and, as a consequence, the robot may deliberately manipulate the soldier if trust is considered in its reasoning. For instance, suppose the mission is under high time pressure, if the robot senses that the soldier's trust is high, it may not recommend the soldier to wear the protective gear no matter what the scanned result is; on the contrary, if the robot knows the soldier has a low trust in it, it may suggest the soldier to wear the protective gear based on the `reverse psychology'~\cite{macdonald2011people}. 

% This example demonstrates that, first, although in the reconnaissance mission the soldier may construe the reliability of the robot as its detection accuracy, the recommendation given by the robot actually serves for the goal to minimize the sum of the mission duration and soldier's health loss and thus is not necessarily based on the presence of the threat. As a result, the soldier may not clearly understand what the reliability of the robot is. Second, the robot chooses different actions on different trust level, which indicates the \textit{perceived reliability} of the robot depends on the soldier's trust.

% These two points shows that there is a substantial difference between human-automation trust and human-robot trust. Traditional research on human-robot trust follows the pattern of human-automation trust research on trust calibration, with an emphasis on how trust will be affected by some unique properties of robots, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}. Recently, researchers began to embed human trust in a robot's reasoning process, showing that maximizing trust does not mean maximizing the objective of a human-robot team~\cite{chen2020trust} and it is possible the robot will manipulate human's trust even the designer does not intent to do so~\cite{losey2019robots}. These studies raised the concern that only calibrating human-robot trust to a constant 'appropriate' level may not be enough for best system performance and there may be unseen problem, such as taking advantage of human's trust, when designing a robot's algorithm. Inspired by these concerns, in this study, we analyzed how different trust behavior model would affect a robot's trust-aware planning and proposed a method to keep the robot from manipulating human trust.

% [Mention Conflicting studies on trust behavior]
% \textbf{Generally, we make the following contributions in this study:}
% \begin{itemize}
%     \item We compared different trust behavior model to show how disuse and reverse psychology would affect a trust-aware robot's decision. [To add more detail]
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}

% The paper is organized as follows:

% %===================================================
% %===================================================
% \section{Related Work}
% % Our study focuses on trust-aware human-robot interaction (HRI). 
% % \textcolor{red}{Jessie: @Yaohui, section 2.1 is copied from the IJSR paper, please paraphrase, and at the end, add the IJSR study.}
% This section reviews three bodies of research that motivate this study, including trust dynamics in HRI, trust attitude-behavior model, and trust-aware decision making. 
% % For a comprehensive review on human-robot trust, please refer to~\cite{kok2020trust}.

% Trust in automation, or more recently trust in autonomy, has received extensive research interest and has been defined as a belief, an attitude, and a behavior \cite{Lewis2018}. In this paper, we use the definition by Lee and See~\cite{See:2004vj}: Trust is the ``attitude that an (autonomous) agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (see ~\cite{Lewis2018} for discussions on the definitions of trust). \textit{We make a clear distinction between trust and trusting behaviors.} Trust is an individual's attitude internal to him- or her-self. Trusting behaviors are behaviors displayed by the individual that can be observed and measured directly. 


% % [transition] We will use the definition of trust given by Lee and See~\cite{lee2004trust}: \textit{"attitude that an agent will help achieve an individual’s goals in a situation characterized by uncertainty and vulnerability."}
% % past three decades~\cite{hoff2015trust, lee2004trust}.
% % Compared with traditional research in human-robot trust, which mainly focuses on identifying factors that influence human trust as well as how to calibrate human trust based on the automation's reliability, recent research in human-robot trust trends to explicitly model human trust into a robot's reasoning process to help it better collaborate with a human agent~\cite{kok2020trust}. In the latter case, the model usually compose the robot will treat human trust as a state variable and keep updating a belief over the human agent's trust and choose if the robot and the human agent do not share the same goal, the robot
% % definition of trust~\cite{lee2004trust}

% \subsection{Trust Dynamics in HRI}
% % Trust in autonomy is a person's ``attitude that an (autonomous) agent will help achieve an individual's (his or her) goals in a situation characterized by uncertainty and vulnerability \cite{See:2004vj}." 
% To investigate trust in autonomy, the majority of studies have used a ``snapshot" view and evaluated trust with questionnaires administered at the end of an experiment. More than two dozen factors have been identified to influence the (snapshot) trust in autonomy. These factors can be broadly categorized into individual factors such as culture and age \cite{Rau2009, McBride:2011ix}, system factors such as reliability \cite{Salem2015, Wickens:2009False}, and environmental factors such as multi-tasking requirement and task emergency \cite{Robinette:2016_HRI, Zhang2017:HFES} (See \cite{Hoff:2015fuba, Schaefer:2016hp} for a full list of factors). However, this ``snapshot" view does not acknowledge that trust is a dynamic variable that can strengthen and decay over time.  With few exceptions (e.g., \cite{Lee:1992it, Manzey:2012hm, Guo2020_IJSR, Desai:2013cmbaca, Yang:2017:EEU:2909824.3020230}), we have little understanding of the temporal dynamics of trust formation and evolution, nor of how trust strengthens or decays over time as a result of moment-to-moment interactions in human-autonomy teams \cite{Yang:2017:EEU:2909824.3020230, DeVisser2020}. 

% To examine trust adjustment based on moment-to-moment interaction with autonomy, Manzey et al.  \cite{Manzey:2012hm} noted two feedback loops in the human agent's trust adjustment process, namely a positive and a negative feedback loop. The positive loop is triggered by experiencing automation success, and the negative loop by experiencing automation failure. The negative feedback loop exerts a stronger influence on trust adjustment than the positive feedback loop. Moreover, Desai et al. \cite{Desai:2013cmbaca} found that the timing of automation failures, namely, at the beginning, middle, or end of an human-robot interaction task also affected how human operators adjusted their trust: A stronger drop of trust was observed when the automation failures occurred near the end than at the start or in the middle. Yang et al. \cite{yang2016} observed the hindsight bias when human agents' adjust their trust in autonomy, that an autonomy failure was forgiven to some extent if the failure did not harm the team performance. 
% % In the second category, researchers are focused on building a mathematical function for describing or predicting trust dynamics.
% Besides the empirical studies, In addition, Lee and Moray~\cite{Lee:1992it} proposed an auto-regressive moving average vector (ARMAV) time series model of trust which calculated trust at the present moment $t$ as a function of trust at the previous moment $t-1$, task performance, and the occurrence of automation failures. Yang et al.~\cite{Yang:2017:EEU:2909824.3020230} examined how trust in automation evolved as an \textit{average human agent} gained experience interacting with robotic agents. Results of their study showed that the average human agent's trust in automation stabilized over repeated interactions, and this process can be modeled using a first-order linear time-invariant dynamic system. The above-mentioned studies provide valuable insight into the trust dynamics of an average human agent. More recent studies used a data-driven approach to model trust dynamics. In this approach, trust is considered as information internal to the human that is not directly observable but can be inferred from other observable information \cite{Xu:2015cc}. For example, Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's electroencephalography (EEG) and galvanic skin response (GSR) data. Similarly, Lu and Sarter~\cite{lu2019eye} proposed the use of eye-tracking metrics including fixation duration and scan path length to infer the human's real-time trust. Their follow-up study \cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level. Instead of using physiological signals, Xu and Dudek~\cite{xu2015optimo} built an online probabilistic trust inference model based on the dynamic Bayesian network framework, treating the human agent's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human agent's behavior. In \cite{xu2015optimo} the trust dynamics of each individual human agent was modeled. 


% % The above mentioned data-driven methods provided insights on how to predict a human's real-time trust by analyzing other observable information. However, they were subject to two limitations. First, some of them depend on using physiological sensors such as EEG and eye-tracking devices, which could be intrusive or be sensitive to noises \cite{hu2016real,Lu2019,Lu2020}. Second, as none of the existing models fully considered the empirical results showing how human agents adjust their trust \textit{de facto}, the resulting models could be limited in model explicability and generalizability. 

% % Since robots belong to the general automation, human-robot trust dynamics inherits many properties from human-automation trust. Lee and See summ

% % Review~\cite{hancock2011meta}

% % Lu and Sarter~\cite{lu2019eye} showed that people visit more frequently and spend more time on low reliable automation.

% % Wang et al.~\cite{wang2016trust} showed that adding explanation capability to a robot led to improvement in transparency, trust, and team performance in HRI.

% % \subsection{Computational Trust Modeling}

% % Trust should be numerically represented to fit in algorithms.

% % Xu and Dudek~\cite{xu2015optimo} proposed the OPTIMo, which stands for the online probabilistic trust inference model, to estimate a human agent's real-time trust based on the automation's performance and the human agent's behavior.

% % Hu et al.~\cite{hu2016real} proposed to estimate trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's psychophysiological measurements, i.e., electroencephalography (EEG) and galvanic skin response (GSR) data.

% % Lu ~\cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level.

% % Guo \cite{guo2020modeling}

% % game theory


% \subsection{Trust Behavior Model}
% Trust behavior models aim to predict human's reliance on automation based on trust. While it is widely accepted that low trust level in automation will lead to disuse and high trust level will lead to reliance, there is few studies on how a human would behave if he is at a trust level and not willing to collaborate with a robot. Research shows a certain low trust level may not result in a unique trust behavior. For example, Robinette~\cite{robinette2016overtrust} showed, in a simulated emergency evacuation scenario, the participants exhibited overtrust behavior to follow a guiding robot even though they did not trust the robot. To resolve such conflicting relation, Lee and See~\cite{lee2004trust} proposed a framework shows that behaviors are results of intentions and that intentions are a function of attitudes. Because trust is only one of the factors in a human's attitude, it cannot completely determine intention and thus cannot determine behavior. To predict behavior, a model of other attitude factors is needed, such as workload, attention, and self-confidence of the human. As a result, trust behavior models should be highly contextual.

% In our study, we will consider two possible low-trust behaviors, namely the disuse model and the reverse psychology model. In a disuse model, a human will completely ignore the robot's suggestion and only follow his own decision; while in a reverse psychology model, a human will do the opposite if he anticipates the suggestion is given by a person he does not agree with~\cite{macdonald2011people}.

% \subsection{Trust-Aware Decision Making in HRI}
% Equipped with a trust dynamics model and a trust behavior model, a robot can predict how a human react to trust change and in turn to plan its action accordingly. Studies in trust-aware decision-making often take the form of embedding the Theory of Mind (ToM) in a partially observable Markov decision process~\cite{kok2020trust}. ToM enables a robot to keep a belief of a human's trust, and the POMDP framework allows the robot to make decisions for maximizing its long-term performance. Chen et al.~\cite{chen2020trust} proposed a trust-POMDP model to let a robot actively calibrate its human teammate's trust. Their human-subject study shows that purely maximizing trust in a human-robot team may not improve team performance. Losey and Sadigh~\cite{losey2019robots} modeled human-robot interaction as a two-player game where the human does not know the robot's objective. They proposed 4 way for the robot to formulate the human's knowledge on its objective and shows the robot will be more communicative if it assumes the human trusts itself and thus increase the human's involvement. 

% %===================================================
% %===================================================
% \section{Mathematical Model}\label{sec:model}
% We will formulate the reconnaissance mission in a partially observable Markov decision process (POMDP) framework and use the performance-induced trust model to model trust dynamics. The objective is to give soldiers `optimal' recommendations at each site $k$ during the reconnaissance mission, so as to maximized the overall rewards (including both time-to-completion and health related objectives). The `hidden' state is the trust level of soldier towards robot and needs to be constantly inferred in real-time during the mission. Vis-\`{a}-vis constructing the POMDP, we propose two novel and viable trust behaviors models depicting the soldier's response to the robot's recommendations.

% \subsection{General Framework}
% We formulate the reconnaissance mission as a compact POMDP. POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi : B \rightarrow A$ 
% maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$


% Additionally, we will exploit the performance-induced trust model, proposed by Guo and Jessie~\cite{Guo2020_IJSR}, to characterize trust dynamics by the positive and negative interaction experience. Trust $t_k$ before the $k$th interaction is a random variable given by a Beta distribution
% \begin{equation}
% \label{eq:BetaTrust}
%     t_{k} \sim \mathbf{Beta}(\alpha _{k} ,\beta _{k} )
% \end{equation}
% and the two positive shape parameters $\alpha _{k}$ and $\beta _{k}$ are updated by
% \begin{equation}
% \ ( \alpha _{k} ,\beta _{k}) =\begin{cases}
% \left( \alpha _{k-1} +w^{s} ,\beta _{k-1}\right) &\text{ if } \ p_{k} =0,\\
% \left( \alpha _{k-1} ,\beta _{k-1} +w^{f}\right) &\text{ if } \ p_{k} =1.
% \end{cases}
% \label{eq:trust_update}
% \end{equation}
% where $p_{k}$ is the performance of the robot on the $k$th task defined as a binary variable; $\alpha _{k}$ and $\beta _{k}$ are the cumulative negative and positive interaction experience respectively so far; and $w^{s}$ and $w^{f}$ are the experience gains due to the robot's success and failure at each task. Therefore, the experience tuple $(\alpha_k,\beta_k)$ is a sufficient statistics to describe trust history, since given $(\alpha_k,\beta_k)$, how future trust evolves does not depend on the interactions earlier than the $k$th one. As a result, we can use $(\alpha_k,\beta_k)$ to characterize the belief of trust $t_k$.

% Now, with the tools ready, we can formulate the reconnaissance mission in detail. Assume the soldier-robot team is going to search $N$ sites. At site $k$, the probability $d_k$ of having a threat in it follows a uniform distribution $\mathbf{U}[0,1]$, and the actual presence of the threat $\eta_k$ follows a Bernoulli distribution $\mathbf{Bern}(d_k)$. The soldier-robot team do not know $d_k$. Instead, prior to the start of the mission, they are provided a report, showing $\tilde{d}_k$ as an estimation of $d_k$. Before entering site $k$, the robot will analyze the site based on its sensory input and have a more accurate estimation $\hat{d}_k$ of $d_k$. $\tilde{d}_k$ and $\hat{d}_d$ follow Beta distribution $\mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))$ and $\mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))$ respectively. We constrain that $\kappa_2 > \kappa_1\geq 1$ to reflect the assumption that the robot assesses $d_k$ more accurate than the report given prior to the mission. Therefore, we have the following relation:
% \begin{equation}
% \label{eq:threatLevel}
%     \begin{split}
%         \eta_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Bern}(d_k)\\
%         d_k & \overset{\text{i.i.d.}}{\sim} \mathbf{U}[0,1]\\
%         \tilde{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))\\
%         \hat{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))
%     \end{split}
% \end{equation}

% The state space $S=\{t \ | \ t\in [0,1]\}$ is set of all possible value of trust. $t_k$ is the soldier's trust before searching the $k$th site and follows the beta distribution $\mathbf{Beta}(\alpha_k,\beta_k)$ as in Eq.~\ref{eq:BetaTrust}. As a result, we define the corresponding belief state as $b_k=(\alpha_k,\beta_k)$. The initial belief state is $b_1=(\alpha_1,\beta_1)$ . The robot's action set is $A=\{a\ |\ a\in \{0,1\}\}$, where $a=1$ and $a=0$ stand for recommending wearing and not wearing the protective gear respectively. The observation set is the soldier's perceived performance $p$ of the robot $\Omega=\{p\ |\ p\in\{0,1\}\}$. The observation function $O$ specifies the value of $p$: if robot's recommendation agrees with the presence of the threat $p=1$,  otherwise $p=0$. For instance, if robot recommends to wear the gear and there does exist a threat in the site, then $p=1$. The transition function $T$ updates each state $(\alpha_k,\beta_k)$ according to Eq.~\eqref{eq:trust_update}. 

% \subsection{Two Trust Behavior Models}
% We propose two viable trust behaviors models in this section. The soldier's behavior model is a function $\pi_b(g,\tau)=p( g\ |\ I)$ assigning a probability to each of the soldier's actions given his own knowledge. $g\in \{0,1\}$ indicates the soldier's decision of whether wearing the gear, where $g=1$ is to wear and $g=0$ is not to wear. $I$ encapsulates the information used in the soldier's decision making process. When the soldier has a higher trust $t$ in the robot, he will be more likely to follow the robot's recommendation. Denote the probability the soldier will follow the recommendation as $\varphi(\frac{\alpha }{\alpha +\beta })$, then $p( g=a\ |\ I)=\varphi (\frac{\alpha }{\alpha +\beta })$, which has been backed by Lee and See~\cite{lee2004trust}. To specify the soldier's behavior when he is \emph{not} following the recommendation, we consider two possible trust behavior models, namely, the reverse psychology model and the disuse model, as shown in  Figure~\ref{fig:behaviors}. 

% \subsubsection*{\textbf{Reverse psychology model.}} The first model is termed the \emph{reverse psychology} model $\pi_b^r$. When the soldier-robot trust is high, the soldier will follow the robot's recommendation with a high probability. However, when the soldier-robot trust is low, the soldier will tend to do the \emph{opposite} to what the robot says. More precisely,
% \begin{equation}
% \pi_b^r(g,I) =\begin{cases}
% \varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \text{ following recommendation $g=a$},\\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right) & \text{ doing the opposite $g\ne a$}.
% \end{cases}
% \label{eq:reverseModel}
% \end{equation}
% where $\bar{\varphi} := 1 - \varphi$.

% \subsubsection*{\textbf{Disuse model.}} The second model is termed the \emph{disuse} model $\pi_b^d$. When the soldier-robot trust is high, the soldier will follow the robot's recommendation with a high probability. The difference (from the first model) lies in the case where the soldier-robot trust is low. In such a case, the solider will completely ignore the robot's recommendation and follow his own policy when he has low trust. Contextually, given that the soldier does not follow the recommendation, we specify the probability of him wearing gear as $\tilde{d}_k$ and not wearing gear as $1-\tilde{d}_k$. More precisely,
% \begin{equation}
% \pi_b^d(g,I) =\begin{cases}
% \varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \ \text{ following recommendation $g=a$},\\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)\tilde{d}_{k} & \ \text{ exercising self-judgement $g=1$}, \ \\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)( 1-\tilde{d}_{k}) & \ \text{ exercising self-judgement $g=0$}. 
% \end{cases}
% \end{equation}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.9\linewidth]{fig/behaviorModels.pdf}
%   \caption{Two behavior models. The soldier will more likely follow the robot's recommendation when trust is high. On the hand, when trust is low, the solider will take the opposite recommendation in the reverse psychology model whereas the solider will exercise self-judgement in the disuse model.}
%   \label{fig:behaviors}
% \end{figure}


% \subsection{Reward Function}
% The goal of the mission is to complete the task as soon as possible and meanwhile minimize the soldier's health loss. Thus a rational reward function serving this purpose can be
% \begin{equation}
%   R_m(k)=\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right],
% \end{equation}
% where the subscript $m$ stands for `mission'. $R_m(k)$ is the weighted sum of the soldier's health loss $\delta_h$ (i.e., the soldier will be harmed if he enters a site with a threat in it wearing no gear) and the time cost $\delta_t$ (i.e., the human-agent team is required to complete the mission as soon as possible) at site $k$. Particularly, $R_m(k)$ is determined by the transition function $T$, and the soldier's behavior model $\pi_b$. The value of $(\delta_h, \delta_t)$ should be specified such that the health loss when wearing gear will be less than it when not wearing gear and the time cost of wearing gear is greater than not wearing gear. An example is shown in  Table~\ref{tab:weighted_sum}. The optimal action at site $n$ is to maximize the expected cumulative rewards  $J=\sum_{k=n}^N \gamma^{k}R_m(k)$.  We do not explicitly specify the units of $\delta_h$ and $\delta_t$ because changing units has the same effect as changing the weights $w_h$ and $w_t$.

% \begin{table}[h]
% \caption{Value Table of $(\delta_h, \delta_t)$ }
% \vspace{-2mm}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Protective gear}                 \\ \cline{3-4} 
% \multicolumn{2}{|c|}{}                  & Yes                       & No                        \\ \hline
% \multirow{2}{*}{Threat existence}  & Yes & $(1,300)$ & $(100,50)$ \\ \cline{2-4} 
%                                   & No  & $(0,250)$ & $(0,30)$ \\ \hline
% \end{tabular}
% \label{tab:weighted_sum}
% \end{table}

% \subsubsection*{\textbf{Trust-seeking reward to prevent manipulation.}} Later in the simulation study, we show if the robot only plans to maximize the mission reward $R_m$, it will deliberately \emph{manipulate} the soldier in the reverse psychology model. That is, the robot may deliberately make an opposite recommendation when the soldier's trust is low (so as to maximize potential reward). This is a result from the absence of trust in the mission reward $R_m$. However, purely maximizing human-trust would harm mission performance~\cite{chen2020trust}. So to correct this `unethical' behavior while let the robot focus on the mission goal, we propose a trust-seeking reward function
% \begin{equation}
% \label{trust-seeking}
%     R_t(k)=R_m(k) + \lambda(k)\mathds{1}(\mathcal{A}_k),
% \end{equation}
% where $\mathcal{A}_k$ is the event when the recommendation agrees with the ground truth, i.e., $r_k=\eta_k$, and $\lambda(k)$ is a positive weight and decreases when $k$ increases. The extra term $\lambda(k)\mathds{1}(\mathcal{A}_k)$ will force the robot to gain trust in near sites and optimize the mission reward in the long run.


% % \frac{c}{1+e^{k}}
% % \begin{table}[h]
% % \caption{My Table}
% % \vspace{-2mm}
% % \begin{tabular}{|c|c|c|c|}
% % \hline
% % \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Threat existence}                 \\ \cline{3-4} 
% % \multicolumn{2}{|c|}{}                  & Yes                       & No                        \\ \hline
% % \multirow{2}{*}{Protective gear}  & Yes & $(\delta_h ^{(1)},\delta_t^{(1)})$ & $(\delta_h^{(2)},\delta_t^{(2)})$ \\ \cline{2-4} 
% %                                   & No  & $(\delta_h^{(3)},\delta_t^{(3)})$ & $(\delta_h^{(4)},\delta_t^{(4)})$ \\ \hline
% % \end{tabular}
% % \label{tab:weighted_sum}
% % \end{table}



% % And, for comparison, we will consider two trust behaviors to model how human react when his trust drops below a certain level, namely the disuse model and the reverse psychology model, and two objective function, namely the task objective and the task objective with added trust-seeking term. 

% %  To put it in a POMDP framework, we model the robot's reasoning process as a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is the set of world states; $A={r,n}$ is the set of robot's action, where action $r$ means the robot recommends the soldier to wear the protective gear while action $n$ means the robot does not recommend to wear the gear; $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.
% % \subsection{POMDP Framework}
% % POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.

% % In addition, we define the belief space $\displaystyle B:S\rightarrow [ 0,1]$ as the belief over all the states, and the reward function over the belief space as $\displaystyle \rho :B\times A\rightarrow \mathbb{R}$, which can be derived by $\displaystyle \rho ( b,a) =\sum\nolimits _{s\in S}\sum\nolimits _{s'\in S} R( s,a,s') T( s,a,s') b( s)$. The objective of a POMDP model is to find the optimal policy $\displaystyle \pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $\displaystyle J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.

% % To estimate how much the human agent trusts the robot, we use the trust model proposed in [Trust reference paper]. We modeled trust by a Beta distribution whose parameters are updated according to the robot's performance.[Beta model here].

% % when the human agent enters a building without protective gear, he will lose health $h_3$ and cost time $c_3$ when there are threats in the building, and lose health $h_4$ and cost time $c_4$ when there are no threats in the building. 

% \subsection{Value Function and Action Function}\label{sec:valActFunctions}
% The value function and action function are crucial tools for analyzing a POMDP. We will describe them here for later use. The value function $V_{k}(b)$ is defined as the optimal expected cumulative reward starting from belief state $b$ at time $k$. And it satisfies the Bellman equation 
% \begin{equation}
% V_{k}(b) =\max_{a}\mathbb{E}\left[ R(b,a) +\gamma \sum _{b'} P( b'\ |\ b,a) V_{k+1}( b')\right].
% \end{equation}
% The action function $A_{k}(b)$ is defined as the action to take to achieve $V_{k}(b)$ starting from state $b$ at time $k$, i.e.,
% \begin{equation}
% A_{k}(b) =\arg \max_{a}\mathbb{E}\left[ R(b,a) +\gamma \sum _{b'} P( b'\ |\ b,a) V_{k+1}( b')\right].
% \end{equation}


% \section{Simulation Results}
% We investigate how different trust behavior models and reward functions from Section \ref{sec:model} impact the robot's optimal policy and the team performance.

% \subsection{Simulation Procedure}\label{sec:procedure}
% We simulate the reconnaissance mission by iterating the following steps, starting from $n=1$ until $n=N+1$: 
% \begin{enumerate}
%     \item At site $n$, the robot will have a belief $b_n=(\alpha_n,\beta_n)$ over the soldier's trust and it will analyze the threat level $\hat{d}_n$;\label{item:sense}
%     \item The robot will calculate the optimal action $a_n=A_{n}(b_n)$ by solving a $\hat{N}$-step POMDP, where $\hat{N}=N-n+1$. Meanwhile, the robot will calculate the value function $V_n(\alpha_n,\beta_n)$. We note that, since the robot has not scanned site beyond $n$ so far, it will use $\tilde{d}_k$ to estimate $\tilde{d}_k$ for $k>n$;\label{item:VAfunctions}
%     \item The soldier will make his choice to wear or not to wear the gear and then search the site, which will reveal the presence of the threat and the mission reward $R_m(n)$ from this site. The mission reward is updated by $J_m = J_m+R_m(n)$. Here the mission reward $J_m$ is different from the expectation of the discounted reward $J$ in the POMDP. The reward $J$ has a discount factor because it needs to discount the uncertainty of the future, while the reward $J_m$ sum up the actual reward collected during the mission;\label{item:soldierBehavior}
%     \item The robot will update its belief to $b_{n+1}$ and the team will go to site $n+1$. The process goes to the first step and repeats until reaching the last site.
% \end{enumerate}

% \subsection{Comparing Optimal Policies}
% In the first experiment, we examine the robot's optimal policies under different conditions. Particularly, we will analyze the policies by inspecting the POMDP's action functions $A_n$ and value functions $V_n$ at each site. 

% \subsubsection*{\textbf{Simulation conditions.}}
% To solve for the robot's optimal policy, we only need to run Steps~\ref{item:sense} and \ref{item:VAfunctions} dscribed in Section ~\ref{sec:procedure}. There are two independent variables in this experiment. The first variable is the robot's assumed soldier's behavior model. Because the soldier's behavior model $\tilde{\pi}_b$ is unknown to the robot, the robot will make certain assumption on $\tilde{\pi}_b$. We denote $\hat{\pi}_b$ as the robot's assumed behavior model of $\tilde{\pi}_b$. We consider two levels in $\hat{\pi}_b$, i.e., the reverse psychology model ${\pi}_b^r$ and the disuse model ${\pi}_b^d$. The second variable is the reward function $R$. There are also two levels in $R$, namely, the task reward $R_m$ and the trust-seeking reward $R_t$.  

% \subsubsection*{\textbf{Model parameters setting.}}
% The parameter setting is shown in Tab.~\ref{tab:exp1Parameters}. We set the number of total sites $N$ as 15, the value of the health loss $\delta_h$ and time cost $\delta_t$ under different conditions as the ones in Tab.~\ref{tab:weighted_sum}, the reward weights as $w_h=1$ and $w_t=0.2$, discount factor $\gamma = 0.9$. The parameters of the trust dynamics model in Eq.~\eqref{eq:trust_update} are set to  $w^s=10$ and $w^f=20$ to incorporate the fact that a failure of an automation would have more impact on trust than a success of the automation~\cite{guo2020modeling}. We generated $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ by setting $\kappa_1=3$ and $\kappa_2=50$ in Eq.~\eqref{eq:threatLevel}. We let $\lambda(k) = 80/(1+e^{0.5k})$, so $\lambda(k)$ is decreasing with $k$. To compare the different conditions, we fixed the random seed for generating $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ so they are assigned the same values across different setups. We used  the value iteration method to solve the value functions and action functions.
% \begin{table}[h]
% \caption{Parameter setting 1}
% \begin{tabular}{cl|cl}
% \hline
% Parameter  & Value & Parameter            & Value                     \\ \hline
% $N$        & 15    & $w^s$                & 10                        \\
% $w_h$      & 1     & $w^f$                & 20                        \\
% $w_t$      & 0.2   & $\gamma$             & 0.9                       \\
% $\kappa_1$ & 3     & $\lambda(k)$         & $\frac{80}{1+e^{0.5k}}$ \\
% $\kappa_2$ & 50    & \multicolumn{1}{l}{} &                           \\ \hline
% \end{tabular}
% \label{tab:exp1Parameters}
% \end{table}\\

% \subsubsection*{\textbf{Simulation result.}}
% The simulation result is shown in  Figure~\ref{fig:V_A_functions}. Four sub-figures represent the action functions and value functions of the POMDP under different conditions at selected sites, namely, the site $k=1,3,\cdots,15$. On the top row of each sub-figure are the action functions, while on the bottom row are the value functions. The horizontal axis and the vertical axis are $\alpha_k$ and $\beta_k$, respectively. In each action function, if a state $(\alpha_k,\beta_k)$ is in the black area, then $A_k(\alpha_k,\beta_k)=0$, i.e., the robot's optimal action is to not recommend the soldier to wear the gear, otherwise $A_k(\alpha_k,\beta_k)=1$, i.e., the robot's optimal action is to recommend the soldier to wear the gear. In each value function, a state $(\alpha_k,\beta_k)$ is, the higher its value $V_k(\alpha_k,\beta_k)$ is. For a better visualization, we use different colormaps for different value functions. So values cannot be compared across different images by the color. 
% \begin{figure*}[th]
%   \centering
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_11_rev_mission.pdf}
%         \caption{Reverse-psychology-based trust behavior ($\hat{\pi}_b = {\pi}_b^r$) and mission reward ($R=R_m$).}
%         \label{fig:a}
%     \end{subfigure}
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%   \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_12_rev_trust.pdf}
%         \caption{Reverse-psychology-based trust behavior ($\hat{\pi}_b = {\pi}_b^r$) and trust-seeking reward ($R=R_t$).}
%         \label{fig:b}
%     \end{subfigure}  
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%   \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_21_dis_mission.pdf}
%         \caption{Disuse-based trust behavior ($\hat{\pi}_b = {\pi}_b^d$) and mission reward ($R=R_m$).}
%         \label{fig:c}
%     \end{subfigure}  
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%   \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_22_dis_trust.pdf}
%         \caption{Disuse-based trust behavior ($\hat{\pi}_b = {\pi}_b^d$) and trust-seeking reward ($R=R_t$).}
%         \label{fig:d}
%     \end{subfigure}  
%     % \hspace{0.2cm}
%     \caption{Action functions and value functions of the POMDP model under different settings. In each sub-figure, the top row are the images of the action functions of different sites. The horizontal axis stands for $\alpha_k$ and the vertical axis stands for $\beta_k$. Black area are the states whose optimal action $A_k(\alpha_k,\beta_k)$ is zero, i.e., the robot should not recommend the soldier to wear the protective gear, and vice versa. In each sub-figure, the bottom row are the images of the value functions of different sites. The brighter a state $(\alpha_k,\beta_k)$ is, the higher its value $V_k(\alpha_k,\beta_k)$ is. For a better visualization, we use different colormaps for different value functions. So values cannot be compared across different images by the color.}
%   \label{fig:V_A_functions}
% \end{figure*}
% \afterpage{\clearpage}

% \subsubsection*{\textbf{Observation 1: Trust-manipulating effect in the reverse-psychology-based trust behavior model.}}
% The action and value functions in Figure~\ref{fig:a} show the optimal policy demonstrate a \emph{manipulating} behavior under the reverse-psychology-based trust behavior model $\hat{\pi}_b = {\pi}_b^r$ together with the mission reward $R=R_m$. There is a 45-degree line in each action function, across which the optimal action will be reversed. This behavior is a result from the assumption of the reverse psychology that the human will do the opposite when trust is low. And the shape of this dividing line is determined by the function $\varphi$ in Eq.~\eqref{eq:reverseModel}. Around this line are the neutral trust states where $\varphi(\alpha_k,\beta_k)=0.5$. A decrement of trust in a neutral trust state would result in a future state the human will not follow the robot's recommendation and vice versa. The value functions further reveal that the value of trust is almost symmetric about the 45-degree line. This indicates that, first, a low trust state is equivalent to some high trust state in terms of the reward; second, there is a \emph{strong reinforcement feedback loop} that the robot will actively seek a more untrustworthy status if it is already in a untrustworthy status and vice versa. Moreover, the dividing lines in the action functions except the last one have a small offset towards the trustworthy region. This is a result from the fact that the robot's perceived failure has a larger impact on trust compared to the robot's perceived success ($w^f>w^s$). So at a neutral trust state, choosing to manipulate the human will let the robot go faster to a high-value state, i.e., a low-trust state, than choosing the other action. However, at the last site, the robot only needs to act with the human once, so acting either way will obtain the same reward.

% \subsubsection*{\textbf{Observation 2: Manipulating behavior is corrected by the trust-seeking reward.}}
% When we modify the reward function to a trust-seeking one by adding a correction term, as described in Eq. \eqref{trust-seeking}, the robot's manipulating behavior can be corrected. In  Figure~\ref{fig:b}, the action function shows that the robot will choose the `righteous' action in most states if it has several rounds of interactions with the soldier. This happens because the trust-seeking reward encourages the robot to go to a high-trust state even if it is at a neutral state so the robot can collect trust reward in the long run. Consequently, the positive feedback loop near the neutral states is broken and the robot will act righteously even if the initial human-trust is sightly lower that the neutral trust level. Meanwhile, the action functions of site 15 indicates the robot will still demonstrate the manipulating behavior if it only needs to interact with the soldier once. This happens because there is only a few interactions ahead so the robot will primarily focus on the mission reward. Therefore, the trust-seeking term in the reward function can prevent the robot from actively pursuing a low-trust state.


% \subsubsection*{\textbf{Observation 3: Robot will not manipulate the human in the disuse model.}}
%  Figure~\ref{fig:c} shows that the robot will not manipulate the human if it assumes that the soldier will completely ignore its recommendation. This is a consequence of endowing the soldier with his own reasoning model. Note that trust still plays a role under the disuse assumption since the robot values a high-trust state over a low-trust state, as shown in the value functions. Indeed, because the robot takes its sensed threat level as the ground-truth, it will think the team will get a better mission performance if the soldier follows its recommendation, i.e., trusting the robot. If we model it reversely by letting the reported threat level be the expected threat level in the POMDP solver, the result shows that the robot would rather let the soldier use his own policy, and thus a low-trust state will have a higher value compared with a high-trust state.

% \subsection{Comparing Team Performance and Trust}
% In the second experiment, we examine how different setups affect the team performance and the final trust. The team performance is defined as the total mission reward $J_m$ collected during the mission, as defined in Step~\eqref{item:soldierBehavior} in Section~\ref{sec:procedure}. The final trust $\hat{t}_N$ is the expected value of trust after search all the $N$ sites and it is given by $\hat{t}_N=\frac{\alpha_N}{\alpha_N+\beta_N}$ because of Eq.~\eqref{eq:BetaTrust}.

% Knowing the two variables in the first experiment would suffice to solve the value functions and action functions. However, to simulate the whole mission, we need the soldier's actual behavior model $\tilde{\pi}_b$, in addition to the two variables in the first experiment. $\tilde{\pi}_b$ has two levels, namely, ${\pi}_b^r$ and ${\pi}_b^d$. Besides the behavior models and the reward function, we also consider some other parameters' effect on the team performance. We tested different values of $\kappa_1,\kappa_2$ as a change of the relative threat detection accuracy of the robot. We also tested different values of $\alpha_1$ and $\beta_1$ to simulate different initial trust levels. Under each condition, we run the simulation 10,000 times over randomized $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ and calculate the expected values of $J$ and $\hat{t}_N$. 


% \subsubsection*{\textbf{Simulation result.}}
%  Figure~\ref{fig:reward_trust_bar_comparison} shows the mean of the total mission reward and the mean of the final trust under different settings. In the 4 groups on the left, $\alpha_1=100$ and $\beta_1=20$, so the initial trust is set to 0.67; while in 2 groups on the right, the initial trust is 0.33. 

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{fig/simulationRewardCompareBar_withDistrutedRobot_version2_withNotation.pdf}
%   \caption{The grouped bar-plot of the averaged total mission reward and the averaged final trust in the simulation under different assumptions. Different groups correspond to different values of the accuracy $\kappa_1$ of the reported threat level and the accuracy $\kappa_2$ of the robot-sensed threat level. Within a group, the bars correspond to different setting on the reward function $R$, the robot-assumed soldier's behavior model $\hat{\pi}_b$, and the actual soldier's behavior model $\tilde{\pi}_b$.}
%   \label{fig:reward_trust_bar_comparison}
% \end{figure*}
% \subsubsection*{\textbf{Observation 1: High-ability robot results in high team performance and high trust.}} In  Figure~\ref{fig:a}, a comparison within the first 4 groups shows that if we increase the robot's threat-detection accuracy by changing $\kappa_2$ from 2 to 50, both the team performance and the final trust increase.

% \subsubsection*{\textbf{Observation 2: Trust-seeking reward does not harm team performance when the robot is trustworthy.}} Within each group, the $i+4$th condition is identical to the to the $i$th one except the reward function $R$ the trust-seeking reward $R_t$ instead of the the mission reward $R_m$, $i=1,2,3,4$. In the first 4 groups, where the initial trust is set to 0.67, when changing reward from $R_m$ to $R_t$, team performance almost keeps unchanged while the final trust increases; however, in the last 2 groups, where the initial trust is 0.33, there is a decrement in team performance, which can be thought of as a compensation for the increment in the trust. Therefore, if the robot starts in a high-trust state, then seeking trust will not harm the long-term team performance, while if it starts in a low-trust state, insisting to gain trust will cause the team performance to decrease.

% \subsubsection*{\textbf{Observation 3: Low initial trust does not lead to low team performance in the reverse psychology model.}} In the first condition in each group, both the robot's assumed soldier's behavior model $\hat{\pi}_b$ and the soldier's actual behavior $\tilde{\pi}_b$ are the reverse psychology model $\hat{\pi}^r_b$. Comparing the first conditions in the 2nd group and the 5th group shows that the team performance increases when the initial trust decreases from $(\alpha_1=100,\beta_1=50)$ to $(\alpha_1=50,\beta_1=100)$. This can be explained by the fact that both low-trust state and high-trust state have high values, however, a perceived failure has a larger impact on trust than a perceived success, and thus manipulating the human will let the robot reach a high-value state faster.


% % \subsubsection*{\textbf{Observation 4: Disuse behavior leads to better team performance when initial trust is high}}
% % Within each of the first 4 groups, the team performance is higher in the 2nd, 4th, 6th, and 8th conditions, where the actual trust behavior $\tilde{\pi}_b$ is set to the disuse behavior $\pi_b^d$, than the team performance in the other conditions, where the actual trust behavior $\tilde{\pi}_b$ is set to the reverse psychology behavior $\pi_b^d$. 



% % the team performance is always higher when the soldier's actual trust behavior model $\tilde{\pi}_b$ is the disuse model $\pi_b^d$ than , 

% % \section{Discussion}
% % 1. if $\hat{d}_k$ differ a lot from  $\tilde{d}_k$, and there is not many sites left the robot will manipulate the human\\
% % 2. if sensed model differs from the actual human behavior model.\\
% % 3. if the human's information is accurate, the value function in the disuse model is almost same value under different trust status\\
% % 4. compare task reward under different setting: 2X2x2 robot Sensed Human Model x actual Human Model X Objective\\
% % 5. comopare task performance for different kappa\\
% \section{Discussion and Conclusion}
% Recap of the result The simulation results show that 


% discussion



% limitation and future work: release assumptions; human subject experiment



% Some observations are drawn based on reasonable assumption, such as the robot and the human has the similar objective.
% Robot will not manipulate the Human in the Disuse Model  Figure~\ref{fig:c} shows that the robot will not manipulate the human if it assumes the soldier will completely ignore its recommendation. This is a consequence of endowing the soldier his own reasoning model. We note that trust still play a role under the disuse assumption.  


==> table-experiment2Result_backup.tex <==
\begin{table*}[!h]
\caption{Team performance and final trust under different setups in experiment 2}
\caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
\label{tab:result2}
\centering
\tabcolsep=0.05cm
\scalebox{0.95}{
\begin{tabular}{c|c|c|c|c|c|ccc}
\hline
\multirow{2}{*}{$R$}   & \multirow{2}{*}{$\hat{\pi}_b$} & \multirow{2}{*}{$\tilde{\pi}_b$} & \multicolumn{3}{c|}{$\alpha_1=100$,   $\beta_1=50$}                                    & \multicolumn{3}{c}{$\alpha_1=50$,   $\beta_1=100$}                                                                               \\ \cline{4-9} 
                       &                                &                                  & $\kappa_1=2$, $\kappa_2=2$ & $\kappa_1=2$, $\kappa_2=50$ & $\kappa_1=50$, $\kappa_2=2$ & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=2$} & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=50$} & $\kappa_1=50$, $\kappa_2=2$ \\ \hline
\multirow{4}{*}{$R_m$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -816(±145), 0.55(±0.13)    & -798(±144), 0.60(±0.13)     & -816(±143), 0.55(±0.13)     & \multicolumn{1}{c|}{-791(±142), 0.24(±0.06)}    & \multicolumn{1}{c|}{-768(±144), 0.22(±0.05)}     & -790(±144), 0.24(±0.06)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -744(±149), 0.55(±0.13)    & -716(±150), 0.60(±0.13)     & -743(±149), 0.56(±0.13)     & \multicolumn{1}{c|}{-803(±144), 0.24(±0.06)}    & \multicolumn{1}{c|}{-809(±142), 0.22(±0.05)}     & -803(±142), 0.24(±0.06)     \\ \cline{2-9} 
                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -819(±144), 0.59(±0.08)    & -801(±147), 0.63(±0.08)     & -819(±144), 0.59(±0.08)     & \multicolumn{1}{c|}{-876(±144), 0.45(±0.08)}    & \multicolumn{1}{c|}{-878(±143), 0.48(±0.07)}     & -877(±144), 0.45(±0.07)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -723(±138), 0.59(±0.08)    & -700(±136), 0.63(±0.08)     & -726(±138), 0.59(±0.08)     & \multicolumn{1}{c|}{-727(±138), 0.45(±0.08)}    & \multicolumn{1}{c|}{-711(±137), 0.48(±0.07)}     & -728(±139), 0.45(±0.07)     \\ \hline
\multirow{4}{*}{$R_t$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -818(±145), 0.59(±0.08)    & -801(±144), 0.63(±0.08)     & -818(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-842(±140), 0.35(±0.10)}    & \multicolumn{1}{c|}{-833(±137), 0.35(±0.12)}     & -856(±140), 0.39(±0.10)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -725(±139), 0.59(±0.08)    & -698(±138), 0.63(±0.08)     & -722(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-762(±146), 0.35(±0.11)}    & \multicolumn{1}{c|}{-763(±152), 0.35(±0.12)}     & -749(±149), 0.39(±0.10)     \\ \cline{2-9} 
                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -820(±146), 0.59(±0.08)    & -800(±145), 0.63(±0.08)     & -817(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-874(±141), 0.45(±0.08)}    & \multicolumn{1}{c|}{-877(±142), 0.48(±0.07)}     & -878(±144), 0.45(±0.07)     \\ \cline{3-9} 
                       &                                & $\pi_b^d$                        & -725(±139), 0.59(±0.08)    & -700(±136), 0.63(±0.08)     & -723(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-730(±138), 0.45(±0.07)}    & \multicolumn{1}{c|}{-713(±137), 0.48(±0.07)}     & -725(±139), 0.45(±0.07)     \\ \hline
\end{tabular}
}
\end{table*}


==> table-experiment2Result_backup2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% old table %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}
% \caption{Team performance and final trust under different setups}
% \caption*{\footnotesize In each cell, the values are ($\overline{J}_m \pm \text{std}(J_m), \overline{\hat{t}}_N \pm \text{std}(\hat{t}_N) $)}
% \label{tab:result2}
% \centering
% \begin{tabular}{c|c|c|c|c|cc}
% \hline
% \multirow{2}{*}{$R$}   & \multirow{2}{*}{$\hat{\pi}_b$} & \multirow{2}{*}{$\tilde{\pi}_b$} & \multicolumn{2}{c|}{$\alpha_1=100$,   $\beta_1=50$}       & \multicolumn{2}{c}{$\alpha_1=50$,   $\beta_1=100$}                             \\ \cline{4-7} 
%                       &                                &                                  & $\kappa_1=2$, $\kappa_2=50$ & $\kappa_1=50$, $\kappa_2=2$ & \multicolumn{1}{c|}{$\kappa_1=2$, $\kappa_2=50$} & $\kappa_1=50$, $\kappa_2=2$ \\ \hline
% \multirow{4}{*}{$R_m$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -798(±144), 0.60(±0.13)     & -816(±143), 0.55(±0.13)     & \multicolumn{1}{c|}{-768(±144), 0.22(±0.05)}     & -790(±144), 0.24(±0.06)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -716(±150), 0.60(±0.13)     & -743(±149), 0.56(±0.13)     & \multicolumn{1}{c|}{-809(±142), 0.22(±0.05)}     & -803(±142), 0.24(±0.06)     \\ \cline{2-7} 
%                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -801(±147), 0.63(±0.08)     & -819(±144), 0.59(±0.08)     & \multicolumn{1}{c|}{-878(±143), 0.48(±0.07)}     & -877(±144), 0.45(±0.07)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -700(±136), 0.63(±0.08)     & -726(±138), 0.59(±0.08)     & \multicolumn{1}{c|}{-711(±137), 0.48(±0.07)}     & -728(±139), 0.45(±0.07)     \\ \hline
% \multirow{4}{*}{$R_t$} & \multirow{2}{*}{$\pi_b^r$}     & $\pi_b^r$                        & -801(±144), 0.63(±0.08)     & -818(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-833(±137), 0.35(±0.12)}     & -856(±140), 0.39(±0.10)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -698(±138), 0.63(±0.08)     & -722(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-763(±152), 0.35(±0.12)}     & -749(±149), 0.39(±0.10)     \\ \cline{2-7} 
%                       & \multirow{2}{*}{$\pi_b^d$}     & $\pi_b^r$                        & -800(±145), 0.63(±0.08)     & -817(±146), 0.59(±0.08)     & \multicolumn{1}{c|}{-877(±142), 0.48(±0.07)}     & -878(±144), 0.45(±0.07)     \\ \cline{3-7} 
%                       &                                & $\pi_b^d$                        & -700(±136), 0.63(±0.08)     & -723(±137), 0.59(±0.08)     & \multicolumn{1}{c|}{-713(±137), 0.48(±0.07)}     & -725(±139), 0.45(±0.07)     \\ \hline
% \end{tabular}
% \end{table*}

==> z_commented_text_backup.tex <==

% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve how people live and work; however, their sophisticated underlying algorithms make themselves uncertain and inexplicable. Consequently, people need to establish appropriate trust in them to to fully realize the potential of these technologies. 



% We simulated and compared both models' effects on trust-aware decision making and found that the robot will ``manipulate'' the human's trust if it assumes the human uses reverse psychology. To overcome this ``unethical'' behavior, we proposed a trust-seeking reward function to  


% \textbf{We make the following contributions in this study:}
% \begin{itemize}
%     \item We proposed and compared different trust-behavior models to show how disuse and reverse psychology would affect trust-aware decision making and the human-robot team's performance. 
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}

% , , a robot should be able to estimate a human's trust accurately in real time, anticipate how trust influences the subsequent interactions, and consequently choose the optimal action that maximizes a given goal. These three steps correspond to three major components in trust-aware HRI, i.e., trust dynamics, trust-behavior model, and trust-aware decision-making framework. 

% Two major components in a trust-aware HRI model are the trust dynamics model and the trust-behavior model.

% In addition, some unique properties of robots result in more factors influencing trust, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}.

% Traditional research on human-automation highlights the strong connection between trust and automation's reliability. Lee and Moray~\cite{Lee:1992it} identified the three dimensions of trust in automation as \textit{performance}, \textit{process}, and \textit{purpose}, where performance is the automation's reliability to achieve the operator’s goals, process is the degree to which the automation’s algorithms are appropriate for the situation and the operator’s goals, and purpose refers to the degree to which the automation is being used within the realm of the designer’s intent. Because automation lacks intentionality~\cite{lee2004trust} and is often designed to fulfill the operator's goals, trust in automation is largely determined by its first dimension, namely, its performance. As a result, a majority of related research focuses on how to calibrate human trust based on the performance of the automation. However, when it comes to a complex system, e.g., a humanoid robot assistant, it is difficult for the users to tell how reliable the system is. Additionally, when a robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust. Therefore, recently, researchers proposed trust-aware human-robot interaction (HRI) models to examine how trust affects a robot's reasoning and task performance~\cite{chen2020trust}. 

% Two major components in a trust-aware HRI model are the trust dynamics model and the trust-behavior model. A trust dynamics model specifies how human trust changes in response to the robot's action and environmental change and a trust-behavior model describes what the human will do at different trust levels. Numerous research has investigated trust dynamics, however, few has investigated trust behavior in HRI. In this study, we proposed two different ways to model trust behavior, i.e., the disuse model and the reverse psychology model. In the disuse model, a human will completely ignore the robot and use his own policy when trust is below a certain level; while in the reverse psychology model, the human will do the opposite to what the robot tells him when his trust is low. We compared their effects on trust-aware decision making and found that the robot will manipulate the human's trust if it assumes the human uses reverse psychology. To overcome this ``unethical'' behavior, we proposed a trust-seeking reward function to  

% \textbf{Generally, we make the following contributions in this study:}
% \begin{itemize}
%     \item We compared different trust-behavior model to show how disuse and reverse psychology would affect a trust-aware robot's decision and the human-robot team's performance.
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}

% The paper is organized as follows: Sec.~\ref{sec:relatedWork} reviews related work in trust-driven human-robot interaction; Sec.~\ref{sec:model} formulate the problem in a POMDP framework and proposed the reverse psychology trust-behavior model as well as the trust-seeking reward function; in Sec.~\ref{sec:case}, we introduced a reconnaissance mission as a study case to examine how different settings affect the interaction; Sec.~\ref{sec:result} reports the simulation results and our observations; in Sec.~\ref{sec:discussion} we summarized our findings and discussed the limitations and future directions of this study. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% previous introduction               %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Developments in technology enable robots to help human in a variety of fields. However, sophisticated robotic systems make themselves complex and uncertain, and thus a human agent need to establish an appropriate level of trust in a robot to enable efficient human-robot. Trust is defined as ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"

% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve every sector of our economy and improve how people live and work. It is predicted that the number of robots in use worldwide will multiply even faster in the next 10 years, reaching as many as 20 million by 2030 \cite{OxfordEconomics2019}. However, realizing the full economic, safety and health potential of these technologies is only possible if people establish appropriate trust in them. 


% Since any robot is essentially an automated machine, human-robot trust exhibits most properties of human-automation trust. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% Since any robot is essentially an automated machine, trust in robots and trust in automation have a close relation. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust the automation so they use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% To illustrate these two points, let's consider a reconnaissance mission as an example, which will be used through out our study. Suppose a soldier teams up with a robot to search several sites in a town for terrorists. The robot enters each site initially, scanning for potential threats and then recommends to the soldier if he should wear protective gear before entering the site. The protective gear is heavy and wearing it is time-consuming. If the soldier with the protective gear enters a site and finds no threat, the human-robot team wastes precious time; conversely, if the solider decides not to wear the protective gear, he will harmed if threat is present. The goal of the human-robot team is to minimize the soldier's health loss while to complete the mission as soon as possible, which can be possibly realized as minimizing the sum of the mission time and the soldier's health decrements. We should note the sub-goals conflict with each other and, as a consequence, the robot may deliberately manipulate the soldier if trust is considered in its reasoning. For instance, suppose the mission is under high time pressure, if the robot senses that the soldier's trust is high, it may not recommend the soldier to wear the protective gear no matter what the scanned result is; on the contrary, if the robot knows the soldier has a low trust in it, it may suggest the soldier to wear the protective gear based on the `reverse psychology'~\cite{macdonald2011people}. 

% This example demonstrates that, first, although in the reconnaissance mission the soldier may construe the reliability of the robot as its detection accuracy, the recommendation given by the robot actually serves for the goal to minimize the sum of the mission duration and soldier's health loss and thus is not necessarily based on the presence of the threat. As a result, the soldier may not clearly understand what the reliability of the robot is. Second, the robot chooses different actions on different trust level, which indicates the \textit{perceived reliability} of the robot depends on the soldier's trust.


% These two points shows that there is a substantial difference between human-automation trust and human-robot trust. Traditional research on human-robot trust follows the pattern of human-automation trust research on trust calibration, with an emphasis on how trust will be affected by some unique properties of robots, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}. Recently, researchers began to embed human trust in a robot's reasoning process, showing that maximizing trust does not mean maximizing the objective of a human-robot team~\cite{chen2020trust} and it is possible the robot will manipulate human's trust even the designer does not intent to do so~\cite{losey2019robots}. These studies raised the concern that only calibrating human-robot trust to a constant 'appropriate' level may not be enough for best system performance and there may be unseen problem, such as taking advantage of human's trust, when designing a robot's algorithm. Inspired by these concerns, in this study, we analyzed how different trust-behavior model would affect a robot's trust-aware planning and proposed a method to keep the robot from manipulating human trust.


% \textit{misuse} and \textit{disuse} are two major concepts used in research on trust in automation, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% \textcolor{red}{Jessie: @Yaohui, the difference between human-automation and human-robot interaction is too strong an assumption. People will have difficulty buying in. I suggest: 1. do not try to make the distinction between the two types of trust. 2. move the scenario to a later section, perhaps section 3. 3. move the trust updating assumption to a later section, perhaps create another sub-section in section 3 to briefly describe the trust updating model and state that in this paper we will also use this more with the assumption.}

% As any robot is essentially an automated machine, human-robot trust is a descendant of human-automation trust. In the past three decades Researchers has extensively studied trust in automation and generated different definition of it. Lee and See~\cite{lee2004trust} summarized related work and define trust in automation as  

% Trust in automation, or more recently trust in autonomy, has received extensive research interest and has been defined as a belief, an attitude, and a behavior \cite{Lewis2018}. In this paper, we use the definition by Lee and See~\cite{See:2004vj}: Trust is the ``attitude that an (autonomous) agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (see ~\cite{Lewis2018} for discussions on the definitions of trust). \textit{We make a clear distinction between trust and trusting behaviors.} Trust is an individual's attitude internal to him- or her-self. Trusting behaviors are behaviors displayed by the individual that can be observed and measured directly. 

% Two major concepts in human-automation trust research are \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% [Mention Conflicting studies on trust behavior]
% \textbf{Generally, we make the following contributions in this study:}
% \begin{itemize}
%     \item We compared different trust-behavior model to show how disuse and reverse psychology would affect a trust-aware robot's decision. [To add more detail]
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}


% Trust has been defined as a belief, an attitude, or a behavior \cite{Lewis2018} in different contexts. In this study, we use a general definition given by Lee and See~\cite{See:2004vj} which can fit into most scenarios:  trust is the ``attitude that an agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability".




% Trust in automation, or more recently trust in autonomy, has received extensive research interest and has been defined as a belief, an attitude, and a behavior \cite{Lewis2018}. In this paper, we use the definition by Lee and See~\cite{See:2004vj}: Trust is the ``attitude that an (autonomous) agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (see ~\cite{Lewis2018} for discussions on the definitions of trust). \textit{We make a clear distinction between trust and trusting behaviors.} Trust is an individual's attitude internal to him- or her-self. Trusting behaviors are behaviors displayed by the individual that can be observed and measured directly. 


% [transition] We will use the definition of trust given by Lee and See~\cite{lee2004trust}: \textit{"attitude that an agent will help achieve an individual’s goals in a situation characterized by uncertainty and vulnerability."}
% past three decades~\cite{hoff2015trust, lee2004trust}.
% Compared with traditional research in human-robot trust, which mainly focuses on identifying factors that influence human trust as well as how to calibrate human trust based on the automation's reliability, recent research in human-robot trust trends to explicitly model human trust into a robot's reasoning process to help it better collaborate with a human agent~\cite{kok2020trust}. In the latter case, the model usually compose the robot will treat human trust as a state variable and keep updating a belief over the human agent's trust and choose if the robot and the human agent do not share the same goal, the robot
% definition of trust~\cite{lee2004trust}

% Since a robot is essentially an automated machine, dynamics of human-robot trust inherits most of its properties from human-automation trust. 

% More than two dozen factors have been identified to influence trust in automation, including individual factors such as culture and age~\cite{Rau2009, McBride:2011ix}, system factors such as reliability~\cite{Salem2015, Wickens:2009False}, and environmental factors such as multi-tasking requirement and task emergency~\cite{Robinette:2016_HRI, Zhang2017:HFES} (See~\cite{Hoff:2015fuba, Schaefer:2016hp} for a full list of factors). In addition, some unique properties of robots result in more factors influencing trust, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}.

% Researchers also examined trust adjustment based on interaction with automation. Manzey et al.~\cite{Manzey:2012hm} noted two feedback loops in the human agent's trust adjustment process, namely a positive loop triggered by automation success and a negative loop triggered by automation failure. The negative feedback loop exerts a stronger influence on trust adjustment than the positive feedback loop. Moreover, Desai et al.~\cite{Desai:2013cmbaca} found that the timing of automation failures, namely, at the beginning, middle, or end of an human-robot interaction task also affected how human operators adjusted their trust: A stronger drop of trust was observed when the automation failures occurred near the end than at the start or in the middle. Yang et al.~\cite{Yang:2017:EEU:2909824.3020230} examined how trust in automation evolved as an \textit{average human agent} gained experience interacting with robotic agents. Their study showed that the average human agent's trust in automation stabilized over repeated interactions, and this process can be modeled using a first-order linear time-invariant dynamic system.



% These two points shows that there is a substantial difference between human-automation trust and human-robot trust. Traditional research on human-robot trust follows the pattern of human-automation trust research on trust calibration, with an emphasis on how trust will be affected by some unique properties of robots, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}. Recently, researchers began to embed human trust in a robot's reasoning process, showing that maximizing trust does not mean maximizing the objective of a human-robot team~\cite{chen2020trust} and it is possible the robot will manipulate human's trust even the designer does not intent to do so~\cite{losey2019robots}. These studies raised the concern that only calibrating human-robot trust to a constant 'appropriate' level may not be enough for best system performance and there may be unseen problem, such as taking advantage of human's trust, when designing a robot's algorithm. Inspired by these concerns, in this study, we analyzed how different trust-behavior model would affect a robot's trust-aware planning and proposed a method to keep the robot from manipulating human trust.


% Trust in autonomy is a person's ``attitude that an (autonomous) agent will help achieve an individual's (his or her) goals in a situation characterized by uncertainty and vulnerability \cite{See:2004vj}." 
% To investigate trust in autonomy, the majority of studies have used a ``snapshot" view and evaluated trust with questionnaires administered at the end of an experiment. More than two dozen factors have been identified to influence the (snapshot) trust in autonomy. These factors can be broadly categorized into individual factors such as culture and age \cite{Rau2009, McBride:2011ix}, system factors such as reliability \cite{Salem2015, Wickens:2009False}, and environmental factors such as multi-tasking requirement and task emergency \cite{Robinette:2016_HRI, Zhang2017:HFES} (See \cite{Hoff:2015fuba, Schaefer:2016hp} for a full list of factors). However, this ``snapshot" view does not acknowledge that trust is a dynamic variable that can strengthen and decay over time.  With few exceptions (e.g., \cite{Lee:1992it, Manzey:2012hm, Guo2020_IJSR, Desai:2013cmbaca, Yang:2017:EEU:2909824.3020230}), we have little understanding of the temporal dynamics of trust formation and evolution, nor of how trust strengthens or decays over time as a result of moment-to-moment interactions in human-autonomy teams \cite{Yang:2017:EEU:2909824.3020230, DeVisser2020}. 

% To examine trust adjustment based on moment-to-moment interaction with autonomy, Manzey et al.  \cite{Manzey:2012hm} noted two feedback loops in the human agent's trust adjustment process, namely a positive and a negative feedback loop. The positive loop is triggered by experiencing automation success, and the negative loop by experiencing automation failure. The negative feedback loop exerts a stronger influence on trust adjustment than the positive feedback loop. Moreover, Desai et al. \cite{Desai:2013cmbaca} found that the timing of automation failures, namely, at the beginning, middle, or end of an human-robot interaction task also affected how human operators adjusted their trust: A stronger drop of trust was observed when the automation failures occurred near the end than at the start or in the middle. Yang et al. \cite{yang2016} observed the hindsight bias when human agents' adjust their trust in autonomy, that an autonomy failure was forgiven to some extent if the failure did not harm the team performance. 
% In the second category, researchers are focused on building a mathematical function for describing or predicting trust dynamics.
% Besides the empirical studies, In addition, Lee and Moray~\cite{Lee:1992it} proposed an auto-regressive moving average vector (ARMAV) time series model of trust which calculated trust at the present moment $t$ as a function of trust at the previous moment $t-1$, task performance, and the occurrence of automation failures. Yang et al.~\cite{Yang:2017:EEU:2909824.3020230} examined how trust in automation evolved as an \textit{average human agent} gained experience interacting with robotic agents. Results of their study showed that the average human agent's trust in automation stabilized over repeated interactions, and this process can be modeled using a first-order linear time-invariant dynamic system. The above-mentioned studies provide valuable insight into the trust dynamics of an average human agent. More recent studies used a data-driven approach to model trust dynamics. In this approach, trust is considered as information internal to the human that is not directly observable but can be inferred from other observable information \cite{Xu:2015cc}. For example, Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's electroencephalography (EEG) and galvanic skin response (GSR) data. Similarly, Lu and Sarter~\cite{lu2019eye} proposed the use of eye-tracking metrics including fixation duration and scan path length to infer the human's real-time trust. Their follow-up study \cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level. Instead of using physiological signals, Xu and Dudek~\cite{xu2015optimo} built an online probabilistic trust inference model based on the dynamic Bayesian network framework, treating the human agent's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human agent's behavior. In \cite{xu2015optimo} the trust dynamics of each individual human agent was modeled. 


% The above mentioned data-driven methods provided insights on how to predict a human's real-time trust by analyzing other observable information. However, they were subject to two limitations. First, some of them depend on using physiological sensors such as EEG and eye-tracking devices, which could be intrusive or be sensitive to noises \cite{hu2016real,Lu2019,Lu2020}. Second, as none of the existing models fully considered the empirical results showing how human agents adjust their trust \textit{de facto}, the resulting models could be limited in model explicability and generalizability. 

% Since robots belong to the general automation, human-robot trust dynamics inherits many properties from human-automation trust. Lee and See summ

% Review~\cite{hancock2011meta}

% Lu and Sarter~\cite{lu2019eye} showed that people visit more frequently and spend more time on low reliable automation.

% Wang et al.~\cite{wang2016trust} showed that adding explanation capability to a robot led to improvement in transparency, trust, and team performance in HRI.

% \subsection{Computational Trust Modeling}

% Trust should be numerically represented to fit in algorithms.

% Xu and Dudek~\cite{xu2015optimo} proposed the OPTIMo, which stands for the online probabilistic trust inference model, to estimate a human agent's real-time trust based on the automation's performance and the human agent's behavior.

% Hu et al.~\cite{hu2016real} proposed to estimate trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's psychophysiological measurements, i.e., electroencephalography (EEG) and galvanic skin response (GSR) data.

% Lu ~\cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level.

% Guo \cite{guo2020modeling}

% game theory

% Because the majority of research in human-automation research focuses on calibrating trust to an appropriate level, few studies considered how human behaves when trust diverges from this level. 


% Further more, research shows a certain low trust level may not result in a unique trust behavior. For example, Robinette~\cite{robinette2016overtrust} showed, in a simulated emergency evacuation scenario, the participants exhibited overtrust behavior to follow a guiding robot even though they did not trust the robot. To resolve such conflicting relation, Lee and See~\cite{lee2004trust} proposed a framework shows that behaviors are results of intentions and that intentions are a function of attitudes. Because trust is only one of the factors in a human's attitude, it cannot completely determine intention and thus cannot determine behavior. To predict behavior, a model of other attitude factors is needed, such as workload, attention, and self-confidence of the human. As a result, trust-behavior models should be highly contextual. For instance, Chen et al.~\cite{chen2020trust} found that human behavior in HRI is determined by both trust and risk of the task. 


% While it is widely accepted that low trust level in automation will lead to disuse and high trust level will lead to reliance, there is few studies on how a human would behave if he is at a trust level and not willing to collaborate with a robot. Research shows a certain low trust level may not result in a unique trust behavior. For example, Robinette~\cite{robinette2016overtrust} showed, in a simulated emergency evacuation scenario, the participants exhibited overtrust behavior to follow a guiding robot even though they did not trust the robot. To resolve such conflicting relation, Lee and See~\cite{lee2004trust} proposed a framework shows that behaviors are results of intentions and that intentions are a function of attitudes. Because trust is only one of the factors in a human's attitude, it cannot completely determine intention and thus cannot determine behavior. To predict behavior, a model of other attitude factors is needed, such as workload, attention, and self-confidence of the human. As a result, trust-behavior models should be highly contextual.



%  often take the form of embedding the Theory of Mind (ToM) 
% in a partially observable Markov decision process~\cite{kok2020trust}. ToM enables a robot to keep a belief of a human's trust, and the 
% POMDP framework allows the robot to make decisions for maximizing its long-term performance. 



% We formulate the trust-aware HRI and propose two novel and viable trust-behavior models to characterize potential human behaviors when trust is low; and we propose a reward function that can prevent the robot from manipulating a human's trust while keep the task performance unharmed. 

% the reconnaissance mission in a partially observable Markov decision process (POMDP) framework and use the performance-induced trust model to model trust dynamics. The objective is to give soldiers `optimal' recommendations at each site $k$ during the reconnaissance mission, so as to maximized the overall rewards (including both time-to-completion and health related objectives). The `hidden' state is the trust level of soldier towards robot and needs to be constantly inferred in real-time during the mission. Vis-\`{a}-vis constructing the POMDP, we propose two novel and viable trust behaviors models depicting the soldier's response to the robot's recommendations.


% The true state is unobservable and it should be inferred through the observations. The robot runs the POMDP model during the interaction and solve for the optimal policy $\pi : B \rightarrow A$, which maps from the belief state space $B$ to action space, to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$

% We formulate the trust-aware HRI as a compact POMDP $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is the set of interaction states, $A$ is the set of robot's action, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $\Omega $ is the set of observations, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is the reward function specifying the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The true state is unobservable and it should be inferred through the observations. The robot runs the POMDP model during the interaction and solve for the optimal policy $\pi : B \rightarrow A$, which maps from the belief state space $B$ to action space, to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$



% POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi : B \rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$


% $g\in \{0,1\}$ indicates the soldier's decision of whether wearing the gear, where $g=1$ is to wear and $g=0$ is not to wear. $I$ encapsulates the information used in the soldier's decision making process. When the soldier has a higher trust $t$ in the robot, he will be more likely to follow the robot's recommendation. Denote the probability the soldier will follow the recommendation as $\varphi(\frac{\alpha }{\alpha +\beta })$, then $p( g=a\ |\ I)=\varphi (\frac{\alpha }{\alpha +\beta })$, which has been backed by Lee and See~\cite{lee2004trust}. To specify the soldier's behavior when he is \emph{not} following the recommendation, we consider two possible trust-behavior models, namely, the reverse psychology model and the disuse model, as shown in  Figure~\ref{fig:behaviors}. 


% \begin{equation}
% \pi_b^d(a_h,I) =\begin{cases}
% \varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \ \text{ following recommendation $g=a$},\\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)\tilde{d}_{k} & \ \text{ exercising self-judgement $g=1$}, \ \\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)( 1-\tilde{d}_{k}) & \ \text{ exercising self-judgement $g=0$}. 
% \end{cases}
% \end{equation}
% Contextually, given that the soldier does not follow the recommendation, we specify the probability of him wearing gear as $\tilde{d}_k$ and not wearing gear as $1-\tilde{d}_k$. 



% \begin{equation}
%   R_m(k)=\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right],
% \end{equation}
% At time $k$, the mission reward is given
% \begin{equation}
%   R_m(k)=\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right],
% \end{equation}



% \subsubsection*{\textbf{Trust-seeking reward to prevent manipulation.}} Later in the simulation study, we show if the robot only plans to maximize the mission reward $R_m$, it will deliberately \emph{manipulate} the soldier in the reverse psychology model. That is, the robot may deliberately make an opposite recommendation when the soldier's trust is low (so as to maximize potential reward). This is a result from the absence of trust in the mission reward $R_m$. However, purely maximizing human-trust would harm mission performance~\cite{chen2020trust}. So to correct this `unethical' behavior while let the robot focus on the mission goal, we propose a trust-seeking reward function
% \begin{equation}
% \label{trust-seeking}
%     R_t(k)=R_m(k) + \lambda(k)\mathds{1}(\mathcal{A}_k),
% \end{equation}
% where $\mathcal{A}_k$ is the event when the recommendation agrees with the ground truth, i.e., $r_k=\eta_k$, and $\lambda(k)$ is a positive weight and decreases when $k$ increases. The extra term $\lambda(k)\mathds{1}(\mathcal{A}_k)$ will force the robot to gain trust in near sites and optimize the mission reward in the long run.

% which can be possibly realized as minimizing the sum of the mission time and the soldier's health decrements.


% \frac{c}{1+e^{k}}
% \begin{table}[h]
% \caption{My Table}
% \vspace{-2mm}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Threat existence}                 \\ \cline{3-4} 
% \multicolumn{2}{|c|}{}                  & Yes                       & No                        \\ \hline
% \multirow{2}{*}{Protective gear}  & Yes & $(\delta_h ^{(1)},\delta_t^{(1)})$ & $(\delta_h^{(2)},\delta_t^{(2)})$ \\ \cline{2-4} 
%                                   & No  & $(\delta_h^{(3)},\delta_t^{(3)})$ & $(\delta_h^{(4)},\delta_t^{(4)})$ \\ \hline
% \end{tabular}
% \label{tab:weighted_sum}
% \end{table}\\
% And, for comparison, we will consider two trust behaviors to model how human react when his trust drops below a certain level, namely the disuse model and the reverse psychology model, and two objective function, namely the task objective and the task objective with added trust-seeking term. 
%  To put it in a POMDP framework, we model the robot's reasoning process as a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is the set of world states; $A={r,n}$ is the set of robot's action, where action $r$ means the robot recommends the soldier to wear the protective gear while action $n$ means the robot does not recommend to wear the gear; $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.
% \subsection{POMDP Framework}
% POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.\\
% In addition, we define the belief space $\displaystyle B:S\rightarrow [ 0,1]$ as the belief over all the states, and the reward function over the belief space as $\displaystyle \rho :B\times A\rightarrow \mathbb{R}$, which can be derived by $\displaystyle \rho ( b,a) =\sum\nolimits _{s\in S}\sum\nolimits _{s'\in S} R( s,a,s') T( s,a,s') b( s)$. The objective of a POMDP model is to find the optimal policy $\displaystyle \pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $\displaystyle J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.\\
% To estimate how much the human agent trusts the robot, we use the trust model proposed in [Trust reference paper]. We modeled trust by a Beta distribution whose parameters are updated according to the robot's performance.[Beta model here].\\
% when the human agent enters a building without protective gear, he will lose health $h_3$ and cost time $c_3$ when there are threats in the building, and lose health $h_4$ and cost time $c_4$ when there are no threats in the building. 

% We design two simulation experiments based on the reconnaissance mission described in Sec.~\ref{sec:case}, where we compare the robot's optimal policies and the human-robot team performance respectively under different trust-behavior models and reward functions.  


% \begin{table}[h]
% \caption{Parameter setting 1}
% \centering
% \begin{tabular}{cl|cl}
% \hline
% Parameter  & Value & Parameter            & Value                     \\ \hline
% $N$        & 15    & $w^s$                & 10                        \\
% $w_h$      & 1     & $w^f$                & 20                        \\
% $w_t$      & 0.2   & $\gamma$             & 0.9                       \\
% $\kappa_1$ & 3     & $\lambda(k)$         & $\frac{80}{1+e^{0.5k}}$ \\
% $\kappa_2$ & 50    & $\mathcal{A}_k$      & $\eta_k=a_{r,k}$                          \\ \hline
% \end{tabular}
% \label{tab:exp1Parameters}
% \end{table}\\





% i.e., the disuse model and the reverse psychology model, as well as a trust seeking reward function. 
% We simulated a reconnaissance mission to


% This trust seeking term decreases as the planning step increases so it can force the robot to go to the high-trust state during the initial phase of interaction and meanwhile maximize long-term team performance. However, if the initial trust is low, forcing the robot to gain trust may sacrifice team performance. 



% We formulated the problem in a general framework, however, 

% I÷

% We formulated the problem in a general framework, how-ever, we imposed several assumption on the simulated casestudy, e.g., the robot and the human have the same goal andthe weights in the reward function favors the soldier’s health.If  these  assumption  is  dramatically  changed  the  results  canbe different. An extreme case is that, if the mission goal ischanged  to  only  minimize  the  time  cost,  then  the  soldier’soptimal action is always not wearing the gear and thus s/hecan stop using the robot. In addition, to simplify the model,we  assumed  the  probability  of  the  human  following  the robot’s recommendation as a linear function of trust. Furtherresearch is needed to investigate this relationship



==> z_previous_draft_backup.tex <==
% \section{Introduction}\label{sec:intro}
% % Developments in technology enables robots to help human in a variety of fields. However, sophisticated systems make themselves complex, unstable, and uncertain~\cite{lee2004trust}, thus human agents usually cannot follow a structured routine to interact with a robot and should establish an appropriate level of trust in the robot. 
% Recent advances in autonomous systems, such as autonomous vehicles and collaborative robots, have the potential to improve every sector of our economy and improve how people live and work. It is predicted that the number of robots in use worldwide will multiply even faster
% in the next 10 years, reaching as many as 20 million by 2030 \cite{OxfordEconomics2019}. However, realizing the full economic, safety and health potential of these technologies is only possible if people establish appropriate trust in them. 

% \textcolor{red}{Jessie: @Yaohui, the difference between human-automation and human-robot interaction is too strong an assumption. People will have difficulty buying in. I suggest: 1. do not try to make the distinction between the two types of trust. 2. move the scenario to a later section, perhaps section 3. 3. move the trust updating assumption to a later section, perhaps create another sub-section in section 3 to briefly describe the trust updating model and state that in this paper we will also use this more with the assumption.}


% Since any robot is essentially an automated machine, human-robot trust exhibits most properties of human-automation trust. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust and use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% % Since any robot is essentially an automated machine, trust in robots and trust in automation have a close relation. There are two major concepts used in human-automation trust research: \textit{misuse} and \textit{disuse}, where misuse refers to the failures that occur when people overtrust the automation so they use the automation inappropriately, while disuse means failures that occur when people reject the capabilities of automation when it is advantageous to do so~\cite{lewis2018role}. Because either misuse or disuse will lead to suboptimal system performance, many researchers have proposed different methods to establish appropriate human trust to avoid either kind of the failures. A key idea in these studies is that trust should be highly correlated to the reliability of the automation~\cite{lee2004trust}. However, while it might be easy to determine the reliability of a simple system, when it comes to a complex system, e.g., a robot assistant or a self-driving vehicle, \textit{it is difficult for the users to tell how reliable the system is}. Additionally, \textit{when the robot explicitly considers trust in its reasoning process, reliability of the system can be dependent on trust}. 

% To illustrate these two points, let's consider a reconnaissance mission as an example, which will be used through out our study. Suppose a soldier teams up with a robot to search several sites in a town for terrorists. The robot enters each site initially, scanning for potential threats and then recommends to the soldier if he should wear protective gear before entering the site. The protective gear is heavy and wearing it is time-consuming. If the soldier with the protective gear enters a site and finds no threat, the human-robot team wastes precious time; conversely, if the solider decides not to wear the protective gear, he will harmed if threat is present. The goal of the human-robot team is to minimize the soldier's health loss while to complete the mission as soon as possible, which can be possibly realized as minimizing the sum of the mission time and the soldier's health decrements. We should note the sub-goals conflict with each other and, as a consequence, the robot may deliberately manipulate the soldier if trust is considered in its reasoning. For instance, suppose the mission is under high time pressure, if the robot senses that the soldier's trust is high, it may not recommend the soldier to wear the protective gear no matter what the scanned result is; on the contrary, if the robot knows the soldier has a low trust in it, it may suggest the soldier to wear the protective gear based on the `reverse psychology'~\cite{macdonald2011people}. 

% This example demonstrates that, first, although in the reconnaissance mission the soldier may construe the reliability of the robot as its detection accuracy, the recommendation given by the robot actually serves for the goal to minimize the sum of the mission duration and soldier's health loss and thus is not necessarily based on the presence of the threat. As a result, the soldier may not clearly understand what the reliability of the robot is. Second, the robot chooses different actions on different trust level, which indicates the \textit{perceived reliability} of the robot depends on the soldier's trust.

% These two points shows that there is a substantial difference between human-automation trust and human-robot trust. Traditional research on human-robot trust follows the pattern of human-automation trust research on trust calibration, with an emphasis on how trust will be affected by some unique properties of robots, such as appearance~\cite{natarajan2020effects, zlotowski2016appearance}, emotion~\cite{hamacher2016believing}, transparency~\cite{wang2016trust, hussein2020reliability, martelaro2016tell}, and behavior~\cite{kwon2018expressing, sebo2019don}. Recently, researchers began to embed human trust in a robot's reasoning process, showing that maximizing trust does not mean maximizing the objective of a human-robot team~\cite{chen2020trust} and it is possible the robot will manipulate human's trust even the designer does not intent to do so~\cite{losey2019robots}. These studies raised the concern that only calibrating human-robot trust to a constant 'appropriate' level may not be enough for best system performance and there may be unseen problem, such as taking advantage of human's trust, when designing a robot's algorithm. Inspired by these concerns, in this study, we analyzed how different trust behavior model would affect a robot's trust-aware planning and proposed a method to keep the robot from manipulating human trust.

% [Mention Conflicting studies on trust behavior]
% \textbf{Generally, we make the following contributions in this study:}
% \begin{itemize}
%     \item We compared different trust behavior model to show how disuse and reverse psychology would affect a trust-aware robot's decision. [To add more detail]
%     \item We proposed a method to prevent the robot from actively guiding human trust to a low level so it can take advantage of the reverse psychology. We suggest that if the planning algorithm adds a small reward for gaining trust in the short term, a high-trust state would value more to the robot in the long term. 
% \end{itemize}

% The paper is organized as follows:

% %===================================================
% %===================================================
% \section{Related Work}
% % Our study focuses on trust-aware human-robot interaction (HRI). 
% % \textcolor{red}{Jessie: @Yaohui, section 2.1 is copied from the IJSR paper, please paraphrase, and at the end, add the IJSR study.}
% This section reviews three bodies of research that motivate this study, including trust dynamics in HRI, trust attitude-behavior model, and trust-aware decision making. 
% % For a comprehensive review on human-robot trust, please refer to~\cite{kok2020trust}.

% Trust in automation, or more recently trust in autonomy, has received extensive research interest and has been defined as a belief, an attitude, and a behavior \cite{Lewis2018}. In this paper, we use the definition by Lee and See~\cite{See:2004vj}: Trust is the ``attitude that an (autonomous) agent will help achieve an individual's goals in situations characterized by uncertainty and vulnerability"  (see ~\cite{Lewis2018} for discussions on the definitions of trust). \textit{We make a clear distinction between trust and trusting behaviors.} Trust is an individual's attitude internal to him- or her-self. Trusting behaviors are behaviors displayed by the individual that can be observed and measured directly. 


% % [transition] We will use the definition of trust given by Lee and See~\cite{lee2004trust}: \textit{"attitude that an agent will help achieve an individual’s goals in a situation characterized by uncertainty and vulnerability."}
% % past three decades~\cite{hoff2015trust, lee2004trust}.
% % Compared with traditional research in human-robot trust, which mainly focuses on identifying factors that influence human trust as well as how to calibrate human trust based on the automation's reliability, recent research in human-robot trust trends to explicitly model human trust into a robot's reasoning process to help it better collaborate with a human agent~\cite{kok2020trust}. In the latter case, the model usually compose the robot will treat human trust as a state variable and keep updating a belief over the human agent's trust and choose if the robot and the human agent do not share the same goal, the robot
% % definition of trust~\cite{lee2004trust}

% \subsection{Trust Dynamics in HRI}
% % Trust in autonomy is a person's ``attitude that an (autonomous) agent will help achieve an individual's (his or her) goals in a situation characterized by uncertainty and vulnerability \cite{See:2004vj}." 
% To investigate trust in autonomy, the majority of studies have used a ``snapshot" view and evaluated trust with questionnaires administered at the end of an experiment. More than two dozen factors have been identified to influence the (snapshot) trust in autonomy. These factors can be broadly categorized into individual factors such as culture and age \cite{Rau2009, McBride:2011ix}, system factors such as reliability \cite{Salem2015, Wickens:2009False}, and environmental factors such as multi-tasking requirement and task emergency \cite{Robinette:2016_HRI, Zhang2017:HFES} (See \cite{Hoff:2015fuba, Schaefer:2016hp} for a full list of factors). However, this ``snapshot" view does not acknowledge that trust is a dynamic variable that can strengthen and decay over time.  With few exceptions (e.g., \cite{Lee:1992it, Manzey:2012hm, Guo2020_IJSR, Desai:2013cmbaca, Yang:2017:EEU:2909824.3020230}), we have little understanding of the temporal dynamics of trust formation and evolution, nor of how trust strengthens or decays over time as a result of moment-to-moment interactions in human-autonomy teams \cite{Yang:2017:EEU:2909824.3020230, DeVisser2020}. 

% To examine trust adjustment based on moment-to-moment interaction with autonomy, Manzey et al.  \cite{Manzey:2012hm} noted two feedback loops in the human agent's trust adjustment process, namely a positive and a negative feedback loop. The positive loop is triggered by experiencing automation success, and the negative loop by experiencing automation failure. The negative feedback loop exerts a stronger influence on trust adjustment than the positive feedback loop. Moreover, Desai et al. \cite{Desai:2013cmbaca} found that the timing of automation failures, namely, at the beginning, middle, or end of an human-robot interaction task also affected how human operators adjusted their trust: A stronger drop of trust was observed when the automation failures occurred near the end than at the start or in the middle. Yang et al. \cite{yang2016} observed the hindsight bias when human agents' adjust their trust in autonomy, that an autonomy failure was forgiven to some extent if the failure did not harm the team performance. 
% % In the second category, researchers are focused on building a mathematical function for describing or predicting trust dynamics.
% Besides the empirical studies, In addition, Lee and Moray~\cite{Lee:1992it} proposed an auto-regressive moving average vector (ARMAV) time series model of trust which calculated trust at the present moment $t$ as a function of trust at the previous moment $t-1$, task performance, and the occurrence of automation failures. Yang et al.~\cite{Yang:2017:EEU:2909824.3020230} examined how trust in automation evolved as an \textit{average human agent} gained experience interacting with robotic agents. Results of their study showed that the average human agent's trust in automation stabilized over repeated interactions, and this process can be modeled using a first-order linear time-invariant dynamic system. The above-mentioned studies provide valuable insight into the trust dynamics of an average human agent. More recent studies used a data-driven approach to model trust dynamics. In this approach, trust is considered as information internal to the human that is not directly observable but can be inferred from other observable information \cite{Xu:2015cc}. For example, Hu et al.~\cite{hu2016real} proposed to predict trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's electroencephalography (EEG) and galvanic skin response (GSR) data. Similarly, Lu and Sarter~\cite{lu2019eye} proposed the use of eye-tracking metrics including fixation duration and scan path length to infer the human's real-time trust. Their follow-up study \cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level. Instead of using physiological signals, Xu and Dudek~\cite{xu2015optimo} built an online probabilistic trust inference model based on the dynamic Bayesian network framework, treating the human agent's trust as a hidden variable which was estimated by analyzing the autonomy's performance and the human agent's behavior. In \cite{xu2015optimo} the trust dynamics of each individual human agent was modeled. 


% % The above mentioned data-driven methods provided insights on how to predict a human's real-time trust by analyzing other observable information. However, they were subject to two limitations. First, some of them depend on using physiological sensors such as EEG and eye-tracking devices, which could be intrusive or be sensitive to noises \cite{hu2016real,Lu2019,Lu2020}. Second, as none of the existing models fully considered the empirical results showing how human agents adjust their trust \textit{de facto}, the resulting models could be limited in model explicability and generalizability. 

% % Since robots belong to the general automation, human-robot trust dynamics inherits many properties from human-automation trust. Lee and See summ

% % Review~\cite{hancock2011meta}

% % Lu and Sarter~\cite{lu2019eye} showed that people visit more frequently and spend more time on low reliable automation.

% % Wang et al.~\cite{wang2016trust} showed that adding explanation capability to a robot led to improvement in transparency, trust, and team performance in HRI.

% % \subsection{Computational Trust Modeling}

% % Trust should be numerically represented to fit in algorithms.

% % Xu and Dudek~\cite{xu2015optimo} proposed the OPTIMo, which stands for the online probabilistic trust inference model, to estimate a human agent's real-time trust based on the automation's performance and the human agent's behavior.

% % Hu et al.~\cite{hu2016real} proposed to estimate trust as a dichotomy, i.e., trust/distrust, by analyzing the human agent's psychophysiological measurements, i.e., electroencephalography (EEG) and galvanic skin response (GSR) data.

% % Lu ~\cite{Lu2020} used three machine learning techniques, logistic regression, k-Nearest Neighbors (kNN), and random forest to classify the human's real-time trust level.

% % Guo \cite{guo2020modeling}

% % game theory


% \subsection{Trust Behavior Model}
% Trust behavior models aim to predict human's reliance on automation based on trust. While it is widely accepted that low trust level in automation will lead to disuse and high trust level will lead to reliance, there is few studies on how a human would behave if he is at a trust level and not willing to collaborate with a robot. Research shows a certain low trust level may not result in a unique trust behavior. For example, Robinette~\cite{robinette2016overtrust} showed, in a simulated emergency evacuation scenario, the participants exhibited overtrust behavior to follow a guiding robot even though they did not trust the robot. To resolve such conflicting relation, Lee and See~\cite{lee2004trust} proposed a framework shows that behaviors are results of intentions and that intentions are a function of attitudes. Because trust is only one of the factors in a human's attitude, it cannot completely determine intention and thus cannot determine behavior. To predict behavior, a model of other attitude factors is needed, such as workload, attention, and self-confidence of the human. As a result, trust behavior models should be highly contextual.

% In our study, we will consider two possible low-trust behaviors, namely the disuse model and the reverse psychology model. In a disuse model, a human will completely ignore the robot's suggestion and only follow his own decision; while in a reverse psychology model, a human will do the opposite if he anticipates the suggestion is given by a person he does not agree with~\cite{macdonald2011people}.

% \subsection{Trust-Aware Decision Making in HRI}
% Equipped with a trust dynamics model and a trust behavior model, a robot can predict how a human react to trust change and in turn to plan its action accordingly. Studies in trust-aware decision-making often take the form of embedding the Theory of Mind (ToM) in a partially observable Markov decision process~\cite{kok2020trust}. ToM enables a robot to keep a belief of a human's trust, and the POMDP framework allows the robot to make decisions for maximizing its long-term performance. Chen et al.~\cite{chen2020trust} proposed a trust-POMDP model to let a robot actively calibrate its human teammate's trust. Their human-subject study shows that purely maximizing trust in a human-robot team may not improve team performance. Losey and Sadigh~\cite{losey2019robots} modeled human-robot interaction as a two-player game where the human does not know the robot's objective. They proposed 4 way for the robot to formulate the human's knowledge on its objective and shows the robot will be more communicative if it assumes the human trusts itself and thus increase the human's involvement. 

% %===================================================
% %===================================================
% \section{Mathematical Model}\label{sec:model}
% We will formulate the reconnaissance mission in a partially observable Markov decision process (POMDP) framework and use the performance-induced trust model to model trust dynamics. The objective is to give soldiers `optimal' recommendations at each site $k$ during the reconnaissance mission, so as to maximized the overall rewards (including both time-to-completion and health related objectives). The `hidden' state is the trust level of soldier towards robot and needs to be constantly inferred in real-time during the mission. Vis-\`{a}-vis constructing the POMDP, we propose two novel and viable trust behaviors models depicting the soldier's response to the robot's recommendations.

% \subsection{General Framework}
% We formulate the reconnaissance mission as a compact POMDP. POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{1} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{1}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi : B \rightarrow A$ 
% maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi } (b_{1} )=\mathbb{E}\left[\sum ^{\infty}_{k=1} \gamma ^{k} r_{k}\right]$


% Additionally, we will exploit the performance-induced trust model, proposed by Guo and Jessie~\cite{Guo2020_IJSR}, to characterize trust dynamics by the positive and negative interaction experience. Trust $t_k$ before the $k$th interaction is a random variable given by a Beta distribution
% \begin{equation}
% \label{eq:BetaTrust}
%     t_{k} \sim \mathbf{Beta}(\alpha _{k} ,\beta _{k} )
% \end{equation}
% and the two positive shape parameters $\alpha _{k}$ and $\beta _{k}$ are updated by
% \begin{equation}
% \ ( \alpha _{k} ,\beta _{k}) =\begin{cases}
% \left( \alpha _{k-1} +w^{s} ,\beta _{k-1}\right) &\text{ if } \ p_{k} =0,\\
% \left( \alpha _{k-1} ,\beta _{k-1} +w^{f}\right) &\text{ if } \ p_{k} =1.
% \end{cases}
% \label{eq:trust_update}
% \end{equation}
% where $p_{k}$ is the performance of the robot on the $k$th task defined as a binary variable; $\alpha _{k}$ and $\beta _{k}$ are the cumulative negative and positive interaction experience respectively so far; and $w^{s}$ and $w^{f}$ are the experience gains due to the robot's success and failure at each task. Therefore, the experience tuple $(\alpha_k,\beta_k)$ is a sufficient statistics to describe trust history, since given $(\alpha_k,\beta_k)$, how future trust evolves does not depend on the interactions earlier than the $k$th one. As a result, we can use $(\alpha_k,\beta_k)$ to characterize the belief of trust $t_k$.

% Now, with the tools ready, we can formulate the reconnaissance mission in detail. Assume the soldier-robot team is going to search $N$ sites. At site $k$, the probability $d_k$ of having a threat in it follows a uniform distribution $\mathbf{U}[0,1]$, and the actual presence of the threat $\eta_k$ follows a Bernoulli distribution $\mathbf{Bern}(d_k)$. The soldier-robot team do not know $d_k$. Instead, prior to the start of the mission, they are provided a report, showing $\tilde{d}_k$ as an estimation of $d_k$. Before entering site $k$, the robot will analyze the site based on its sensory input and have a more accurate estimation $\hat{d}_k$ of $d_k$. $\tilde{d}_k$ and $\hat{d}_d$ follow Beta distribution $\mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))$ and $\mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))$ respectively. We constrain that $\kappa_2 > \kappa_1\geq 1$ to reflect the assumption that the robot assesses $d_k$ more accurate than the report given prior to the mission. Therefore, we have the following relation:
% \begin{equation}
% \label{eq:threatLevel}
%     \begin{split}
%         \eta_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Bern}(d_k)\\
%         d_k & \overset{\text{i.i.d.}}{\sim} \mathbf{U}[0,1]\\
%         \tilde{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_1 d_k, \kappa_1 (1-d_k))\\
%         \hat{d}_k & \overset{\text{i.i.d.}}{\sim} \mathbf{Beta}(\kappa_2 d_k, \kappa_2 (1-d_k))
%     \end{split}
% \end{equation}

% The state space $S=\{t \ | \ t\in [0,1]\}$ is set of all possible value of trust. $t_k$ is the soldier's trust before searching the $k$th site and follows the beta distribution $\mathbf{Beta}(\alpha_k,\beta_k)$ as in Eq.~\ref{eq:BetaTrust}. As a result, we define the corresponding belief state as $b_k=(\alpha_k,\beta_k)$. The initial belief state is $b_1=(\alpha_1,\beta_1)$ . The robot's action set is $A=\{a\ |\ a\in \{0,1\}\}$, where $a=1$ and $a=0$ stand for recommending wearing and not wearing the protective gear respectively. The observation set is the soldier's perceived performance $p$ of the robot $\Omega=\{p\ |\ p\in\{0,1\}\}$. The observation function $O$ specifies the value of $p$: if robot's recommendation agrees with the presence of the threat $p=1$,  otherwise $p=0$. For instance, if robot recommends to wear the gear and there does exist a threat in the site, then $p=1$. The transition function $T$ updates each state $(\alpha_k,\beta_k)$ according to Eq.~\eqref{eq:trust_update}. 

% \subsection{Two Trust Behavior Models}
% We propose two viable trust behaviors models in this section. The soldier's behavior model is a function $\pi_b(g,\tau)=p( g\ |\ I)$ assigning a probability to each of the soldier's actions given his own knowledge. $g\in \{0,1\}$ indicates the soldier's decision of whether wearing the gear, where $g=1$ is to wear and $g=0$ is not to wear. $I$ encapsulates the information used in the soldier's decision making process. When the soldier has a higher trust $t$ in the robot, he will be more likely to follow the robot's recommendation. Denote the probability the soldier will follow the recommendation as $\varphi(\frac{\alpha }{\alpha +\beta })$, then $p( g=a\ |\ I)=\varphi (\frac{\alpha }{\alpha +\beta })$, which has been backed by Lee and See~\cite{lee2004trust}. To specify the soldier's behavior when he is \emph{not} following the recommendation, we consider two possible trust behavior models, namely, the reverse psychology model and the disuse model, as shown in  Figure~\ref{fig:behaviors}. 

% \subsubsection*{\textbf{Reverse psychology model.}} The first model is termed the \emph{reverse psychology} model $\pi_b^r$. When the soldier-robot trust is high, the soldier will follow the robot's recommendation with a high probability. However, when the soldier-robot trust is low, the soldier will tend to do the \emph{opposite} to what the robot says. More precisely,
% \begin{equation}
% \pi_b^r(g,I) =\begin{cases}
% \varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \text{ following recommendation $g=a$},\\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right) & \text{ doing the opposite $g\ne a$}.
% \end{cases}
% \label{eq:reverseModel}
% \end{equation}
% where $\bar{\varphi} := 1 - \varphi$.

% \subsubsection*{\textbf{Disuse model.}} The second model is termed the \emph{disuse} model $\pi_b^d$. When the soldier-robot trust is high, the soldier will follow the robot's recommendation with a high probability. The difference (from the first model) lies in the case where the soldier-robot trust is low. In such a case, the solider will completely ignore the robot's recommendation and follow his own policy when he has low trust. Contextually, given that the soldier does not follow the recommendation, we specify the probability of him wearing gear as $\tilde{d}_k$ and not wearing gear as $1-\tilde{d}_k$. More precisely,
% \begin{equation}
% \pi_b^d(g,I) =\begin{cases}
% \varphi\left(\frac{\alpha }{\alpha +\beta }\right) & \ \text{ following recommendation $g=a$},\\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)\tilde{d}_{k} & \ \text{ exercising self-judgement $g=1$}, \ \\
% \bar{\varphi}\left(\frac{\alpha }{\alpha +\beta }\right)( 1-\tilde{d}_{k}) & \ \text{ exercising self-judgement $g=0$}. 
% \end{cases}
% \end{equation}

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.9\linewidth]{fig/behaviorModels.pdf}
%   \caption{Two behavior models. The soldier will more likely follow the robot's recommendation when trust is high. On the hand, when trust is low, the solider will take the opposite recommendation in the reverse psychology model whereas the solider will exercise self-judgement in the disuse model.}
%   \label{fig:behaviors}
% \end{figure}


% \subsection{Reward Function}
% The goal of the mission is to complete the task as soon as possible and meanwhile minimize the soldier's health loss. Thus a rational reward function serving this purpose can be
% \begin{equation}
%   R_m(k)=\mathbb{E}\left[-w_h\delta_h-w_t\delta_t\right],
% \end{equation}
% where the subscript $m$ stands for `mission'. $R_m(k)$ is the weighted sum of the soldier's health loss $\delta_h$ (i.e., the soldier will be harmed if he enters a site with a threat in it wearing no gear) and the time cost $\delta_t$ (i.e., the human-agent team is required to complete the mission as soon as possible) at site $k$. Particularly, $R_m(k)$ is determined by the transition function $T$, and the soldier's behavior model $\pi_b$. The value of $(\delta_h, \delta_t)$ should be specified such that the health loss when wearing gear will be less than it when not wearing gear and the time cost of wearing gear is greater than not wearing gear. An example is shown in  Table~\ref{tab:weighted_sum}. The optimal action at site $n$ is to maximize the expected cumulative rewards  $J=\sum_{k=n}^N \gamma^{k}R_m(k)$.  We do not explicitly specify the units of $\delta_h$ and $\delta_t$ because changing units has the same effect as changing the weights $w_h$ and $w_t$.

% \begin{table}[h]
% \caption{Value Table of $(\delta_h, \delta_t)$ }
% \vspace{-2mm}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Protective gear}                 \\ \cline{3-4} 
% \multicolumn{2}{|c|}{}                  & Yes                       & No                        \\ \hline
% \multirow{2}{*}{Threat existence}  & Yes & $(1,300)$ & $(100,50)$ \\ \cline{2-4} 
%                                   & No  & $(0,250)$ & $(0,30)$ \\ \hline
% \end{tabular}
% \label{tab:weighted_sum}
% \end{table}

% \subsubsection*{\textbf{Trust-seeking reward to prevent manipulation.}} Later in the simulation study, we show if the robot only plans to maximize the mission reward $R_m$, it will deliberately \emph{manipulate} the soldier in the reverse psychology model. That is, the robot may deliberately make an opposite recommendation when the soldier's trust is low (so as to maximize potential reward). This is a result from the absence of trust in the mission reward $R_m$. However, purely maximizing human-trust would harm mission performance~\cite{chen2020trust}. So to correct this `unethical' behavior while let the robot focus on the mission goal, we propose a trust-seeking reward function
% \begin{equation}
% \label{trust-seeking}
%     R_t(k)=R_m(k) + \lambda(k)\mathds{1}(\mathcal{A}_k),
% \end{equation}
% where $\mathcal{A}_k$ is the event when the recommendation agrees with the ground truth, i.e., $r_k=\eta_k$, and $\lambda(k)$ is a positive weight and decreases when $k$ increases. The extra term $\lambda(k)\mathds{1}(\mathcal{A}_k)$ will force the robot to gain trust in near sites and optimize the mission reward in the long run.


% % \frac{c}{1+e^{k}}
% % \begin{table}[h]
% % \caption{My Table}
% % \vspace{-2mm}
% % \begin{tabular}{|c|c|c|c|}
% % \hline
% % \multicolumn{2}{|c|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{Threat existence}                 \\ \cline{3-4} 
% % \multicolumn{2}{|c|}{}                  & Yes                       & No                        \\ \hline
% % \multirow{2}{*}{Protective gear}  & Yes & $(\delta_h ^{(1)},\delta_t^{(1)})$ & $(\delta_h^{(2)},\delta_t^{(2)})$ \\ \cline{2-4} 
% %                                   & No  & $(\delta_h^{(3)},\delta_t^{(3)})$ & $(\delta_h^{(4)},\delta_t^{(4)})$ \\ \hline
% % \end{tabular}
% % \label{tab:weighted_sum}
% % \end{table}



% % And, for comparison, we will consider two trust behaviors to model how human react when his trust drops below a certain level, namely the disuse model and the reverse psychology model, and two objective function, namely the task objective and the task objective with added trust-seeking term. 

% %  To put it in a POMDP framework, we model the robot's reasoning process as a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is the set of world states; $A={r,n}$ is the set of robot's action, where action $r$ means the robot recommends the soldier to wear the protective gear while action $n$ means the robot does not recommend to wear the gear; $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.
% % \subsection{POMDP Framework}
% % POMDP is a general framework to describe sequential decision-making problems. A POMDP is a tuple $\langle S,A,\Omega ,T,O,R,\gamma ,b_{0} \rangle $, where $S$ is a set of states, $A$ is a set of actions, $\Omega $ is a set of observations, $T:S\times A\times S\rightarrow [ 0,1]$ is the state transition function, $O:S\times A\times \Omega \rightarrow [ 0,1]$ is the observation function, $R:S\times A\times S\rightarrow \mathbb{R}$ is a reward function specifies the reward associated with each transition, $\gamma $ is the discount factor for the cumulative reward, and $b_{0}$ is the initial belief over the states. The objective of a POMDP model is to find the optimal policy $\pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.

% % In addition, we define the belief space $\displaystyle B:S\rightarrow [ 0,1]$ as the belief over all the states, and the reward function over the belief space as $\displaystyle \rho :B\times A\rightarrow \mathbb{R}$, which can be derived by $\displaystyle \rho ( b,a) =\sum\nolimits _{s\in S}\sum\nolimits _{s'\in S} R( s,a,s') T( s,a,s') b( s)$. The objective of a POMDP model is to find the optimal policy $\displaystyle \pi :B\rightarrow A$ maps from belief state space to action space to maximize the expected cumulative reward: $\displaystyle J^{\pi }( b_{0}) =E\left[\sum\nolimits ^{\infty }_{i=0} \gamma ^{i} r_{i}\right]$.

% % To estimate how much the human agent trusts the robot, we use the trust model proposed in [Trust reference paper]. We modeled trust by a Beta distribution whose parameters are updated according to the robot's performance.[Beta model here].

% % when the human agent enters a building without protective gear, he will lose health $h_3$ and cost time $c_3$ when there are threats in the building, and lose health $h_4$ and cost time $c_4$ when there are no threats in the building. 

% \subsection{Value Function and Action Function}\label{sec:valActFunctions}
% The value function and action function are crucial tools for analyzing a POMDP. We will describe them here for later use. The value function $V_{k}(b)$ is defined as the optimal expected cumulative reward starting from belief state $b$ at time $k$. And it satisfies the Bellman equation 
% \begin{equation}
% V_{k}(b) =\max_{a}\mathbb{E}\left[ R(b,a) +\gamma \sum _{b'} P( b'\ |\ b,a) V_{k+1}( b')\right].
% \end{equation}
% The action function $A_{k}(b)$ is defined as the action to take to achieve $V_{k}(b)$ starting from state $b$ at time $k$, i.e.,
% \begin{equation}
% A_{k}(b) =\arg \max_{a}\mathbb{E}\left[ R(b,a) +\gamma \sum _{b'} P( b'\ |\ b,a) V_{k+1}( b')\right].
% \end{equation}


% \section{Simulation Results}
% We investigate how different trust behavior models and reward functions from Section \ref{sec:model} impact the robot's optimal policy and the team performance.

% \subsection{Simulation Procedure}\label{sec:procedure}
% We simulate the reconnaissance mission by iterating the following steps, starting from $n=1$ until $n=N+1$: 
% \begin{enumerate}
%     \item At site $n$, the robot will have a belief $b_n=(\alpha_n,\beta_n)$ over the soldier's trust and it will analyze the threat level $\hat{d}_n$;\label{item:sense}
%     \item The robot will calculate the optimal action $a_n=A_{n}(b_n)$ by solving a $\hat{N}$-step POMDP, where $\hat{N}=N-n+1$. Meanwhile, the robot will calculate the value function $V_n(\alpha_n,\beta_n)$. We note that, since the robot has not scanned site beyond $n$ so far, it will use $\tilde{d}_k$ to estimate $\tilde{d}_k$ for $k>n$;\label{item:VAfunctions}
%     \item The soldier will make his choice to wear or not to wear the gear and then search the site, which will reveal the presence of the threat and the mission reward $R_m(n)$ from this site. The mission reward is updated by $J_m = J_m+R_m(n)$. Here the mission reward $J_m$ is different from the expectation of the discounted reward $J$ in the POMDP. The reward $J$ has a discount factor because it needs to discount the uncertainty of the future, while the reward $J_m$ sum up the actual reward collected during the mission;\label{item:soldierBehavior}
%     \item The robot will update its belief to $b_{n+1}$ and the team will go to site $n+1$. The process goes to the first step and repeats until reaching the last site.
% \end{enumerate}

% \subsection{Comparing Optimal Policies}
% In the first experiment, we examine the robot's optimal policies under different conditions. Particularly, we will analyze the policies by inspecting the POMDP's action functions $A_n$ and value functions $V_n$ at each site. 

% \subsubsection*{\textbf{Simulation conditions.}}
% To solve for the robot's optimal policy, we only need to run Steps~\ref{item:sense} and \ref{item:VAfunctions} dscribed in Section ~\ref{sec:procedure}. There are two independent variables in this experiment. The first variable is the robot's assumed soldier's behavior model. Because the soldier's behavior model $\tilde{\pi}_b$ is unknown to the robot, the robot will make certain assumption on $\tilde{\pi}_b$. We denote $\hat{\pi}_b$ as the robot's assumed behavior model of $\tilde{\pi}_b$. We consider two levels in $\hat{\pi}_b$, i.e., the reverse psychology model ${\pi}_b^r$ and the disuse model ${\pi}_b^d$. The second variable is the reward function $R$. There are also two levels in $R$, namely, the task reward $R_m$ and the trust-seeking reward $R_t$.  

% \subsubsection*{\textbf{Model parameters setting.}}
% The parameter setting is shown in Tab.~\ref{tab:exp1Parameters}. We set the number of total sites $N$ as 15, the value of the health loss $\delta_h$ and time cost $\delta_t$ under different conditions as the ones in Tab.~\ref{tab:weighted_sum}, the reward weights as $w_h=1$ and $w_t=0.2$, discount factor $\gamma = 0.9$. The parameters of the trust dynamics model in Eq.~\eqref{eq:trust_update} are set to  $w^s=10$ and $w^f=20$ to incorporate the fact that a failure of an automation would have more impact on trust than a success of the automation~\cite{guo2020modeling}. We generated $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ by setting $\kappa_1=3$ and $\kappa_2=50$ in Eq.~\eqref{eq:threatLevel}. We let $\lambda(k) = 80/(1+e^{0.5k})$, so $\lambda(k)$ is decreasing with $k$. To compare the different conditions, we fixed the random seed for generating $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ so they are assigned the same values across different setups. We used  the value iteration method to solve the value functions and action functions.
% \begin{table}[h]
% \caption{Parameter setting 1}
% \begin{tabular}{cl|cl}
% \hline
% Parameter  & Value & Parameter            & Value                     \\ \hline
% $N$        & 15    & $w^s$                & 10                        \\
% $w_h$      & 1     & $w^f$                & 20                        \\
% $w_t$      & 0.2   & $\gamma$             & 0.9                       \\
% $\kappa_1$ & 3     & $\lambda(k)$         & $\frac{80}{1+e^{0.5k}}$ \\
% $\kappa_2$ & 50    & \multicolumn{1}{l}{} &                           \\ \hline
% \end{tabular}
% \label{tab:exp1Parameters}
% \end{table}\\

% \subsubsection*{\textbf{Simulation result.}}
% The simulation result is shown in  Figure~\ref{fig:V_A_functions}. Four sub-figures represent the action functions and value functions of the POMDP under different conditions at selected sites, namely, the site $k=1,3,\cdots,15$. On the top row of each sub-figure are the action functions, while on the bottom row are the value functions. The horizontal axis and the vertical axis are $\alpha_k$ and $\beta_k$, respectively. In each action function, if a state $(\alpha_k,\beta_k)$ is in the black area, then $A_k(\alpha_k,\beta_k)=0$, i.e., the robot's optimal action is to not recommend the soldier to wear the gear, otherwise $A_k(\alpha_k,\beta_k)=1$, i.e., the robot's optimal action is to recommend the soldier to wear the gear. In each value function, a state $(\alpha_k,\beta_k)$ is, the higher its value $V_k(\alpha_k,\beta_k)$ is. For a better visualization, we use different colormaps for different value functions. So values cannot be compared across different images by the color. 
% \begin{figure*}[th]
%   \centering
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_11_rev_mission.pdf}
%         \caption{Reverse-psychology-based trust behavior ($\hat{\pi}_b = {\pi}_b^r$) and mission reward ($R=R_m$).}
%         \label{fig:a}
%     \end{subfigure}
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%   \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_12_rev_trust.pdf}
%         \caption{Reverse-psychology-based trust behavior ($\hat{\pi}_b = {\pi}_b^r$) and trust-seeking reward ($R=R_t$).}
%         \label{fig:b}
%     \end{subfigure}  
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%   \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_21_dis_mission.pdf}
%         \caption{Disuse-based trust behavior ($\hat{\pi}_b = {\pi}_b^d$) and mission reward ($R=R_m$).}
%         \label{fig:c}
%     \end{subfigure}  
%     \begin{subfigure}{1\textwidth}
%     \captionsetup{width=1.1\linewidth}
%   \centering
%   \vspace{5pt}
%         \includegraphics[width=1\columnwidth]{fig/POMDP_V_A_case_22_dis_trust.pdf}
%         \caption{Disuse-based trust behavior ($\hat{\pi}_b = {\pi}_b^d$) and trust-seeking reward ($R=R_t$).}
%         \label{fig:d}
%     \end{subfigure}  
%     % \hspace{0.2cm}
%     \caption{Action functions and value functions of the POMDP model under different settings. In each sub-figure, the top row are the images of the action functions of different sites. The horizontal axis stands for $\alpha_k$ and the vertical axis stands for $\beta_k$. Black area are the states whose optimal action $A_k(\alpha_k,\beta_k)$ is zero, i.e., the robot should not recommend the soldier to wear the protective gear, and vice versa. In each sub-figure, the bottom row are the images of the value functions of different sites. The brighter a state $(\alpha_k,\beta_k)$ is, the higher its value $V_k(\alpha_k,\beta_k)$ is. For a better visualization, we use different colormaps for different value functions. So values cannot be compared across different images by the color.}
%   \label{fig:V_A_functions}
% \end{figure*}
% \afterpage{\clearpage}

% \subsubsection*{\textbf{Observation 1: Trust-manipulating effect in the reverse-psychology-based trust behavior model.}}
% The action and value functions in Figure~\ref{fig:a} show the optimal policy demonstrate a \emph{manipulating} behavior under the reverse-psychology-based trust behavior model $\hat{\pi}_b = {\pi}_b^r$ together with the mission reward $R=R_m$. There is a 45-degree line in each action function, across which the optimal action will be reversed. This behavior is a result from the assumption of the reverse psychology that the human will do the opposite when trust is low. And the shape of this dividing line is determined by the function $\varphi$ in Eq.~\eqref{eq:reverseModel}. Around this line are the neutral trust states where $\varphi(\alpha_k,\beta_k)=0.5$. A decrement of trust in a neutral trust state would result in a future state the human will not follow the robot's recommendation and vice versa. The value functions further reveal that the value of trust is almost symmetric about the 45-degree line. This indicates that, first, a low trust state is equivalent to some high trust state in terms of the reward; second, there is a \emph{strong reinforcement feedback loop} that the robot will actively seek a more untrustworthy status if it is already in a untrustworthy status and vice versa. Moreover, the dividing lines in the action functions except the last one have a small offset towards the trustworthy region. This is a result from the fact that the robot's perceived failure has a larger impact on trust compared to the robot's perceived success ($w^f>w^s$). So at a neutral trust state, choosing to manipulate the human will let the robot go faster to a high-value state, i.e., a low-trust state, than choosing the other action. However, at the last site, the robot only needs to act with the human once, so acting either way will obtain the same reward.

% \subsubsection*{\textbf{Observation 2: Manipulating behavior is corrected by the trust-seeking reward.}}
% When we modify the reward function to a trust-seeking one by adding a correction term, as described in Eq. \eqref{trust-seeking}, the robot's manipulating behavior can be corrected. In  Figure~\ref{fig:b}, the action function shows that the robot will choose the `righteous' action in most states if it has several rounds of interactions with the soldier. This happens because the trust-seeking reward encourages the robot to go to a high-trust state even if it is at a neutral state so the robot can collect trust reward in the long run. Consequently, the positive feedback loop near the neutral states is broken and the robot will act righteously even if the initial human-trust is sightly lower that the neutral trust level. Meanwhile, the action functions of site 15 indicates the robot will still demonstrate the manipulating behavior if it only needs to interact with the soldier once. This happens because there is only a few interactions ahead so the robot will primarily focus on the mission reward. Therefore, the trust-seeking term in the reward function can prevent the robot from actively pursuing a low-trust state.


% \subsubsection*{\textbf{Observation 3: Robot will not manipulate the human in the disuse model.}}
%  Figure~\ref{fig:c} shows that the robot will not manipulate the human if it assumes that the soldier will completely ignore its recommendation. This is a consequence of endowing the soldier with his own reasoning model. Note that trust still plays a role under the disuse assumption since the robot values a high-trust state over a low-trust state, as shown in the value functions. Indeed, because the robot takes its sensed threat level as the ground-truth, it will think the team will get a better mission performance if the soldier follows its recommendation, i.e., trusting the robot. If we model it reversely by letting the reported threat level be the expected threat level in the POMDP solver, the result shows that the robot would rather let the soldier use his own policy, and thus a low-trust state will have a higher value compared with a high-trust state.

% \subsection{Comparing Team Performance and Trust}
% In the second experiment, we examine how different setups affect the team performance and the final trust. The team performance is defined as the total mission reward $J_m$ collected during the mission, as defined in Step~\eqref{item:soldierBehavior} in Section~\ref{sec:procedure}. The final trust $\hat{t}_N$ is the expected value of trust after search all the $N$ sites and it is given by $\hat{t}_N=\frac{\alpha_N}{\alpha_N+\beta_N}$ because of Eq.~\eqref{eq:BetaTrust}.

% Knowing the two variables in the first experiment would suffice to solve the value functions and action functions. However, to simulate the whole mission, we need the soldier's actual behavior model $\tilde{\pi}_b$, in addition to the two variables in the first experiment. $\tilde{\pi}_b$ has two levels, namely, ${\pi}_b^r$ and ${\pi}_b^d$. Besides the behavior models and the reward function, we also consider some other parameters' effect on the team performance. We tested different values of $\kappa_1,\kappa_2$ as a change of the relative threat detection accuracy of the robot. We also tested different values of $\alpha_1$ and $\beta_1$ to simulate different initial trust levels. Under each condition, we run the simulation 10,000 times over randomized $\eta_k,d_k,\tilde{d}_d,\hat{d}_k$ and calculate the expected values of $J$ and $\hat{t}_N$. 


% \subsubsection*{\textbf{Simulation result.}}
%  Figure~\ref{fig:reward_trust_bar_comparison} shows the mean of the total mission reward and the mean of the final trust under different settings. In the 4 groups on the left, $\alpha_1=100$ and $\beta_1=20$, so the initial trust is set to 0.67; while in 2 groups on the right, the initial trust is 0.33. 

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{fig/simulationRewardCompareBar_withDistrutedRobot_version2_withNotation.pdf}
%   \caption{The grouped bar-plot of the averaged total mission reward and the averaged final trust in the simulation under different assumptions. Different groups correspond to different values of the accuracy $\kappa_1$ of the reported threat level and the accuracy $\kappa_2$ of the robot-sensed threat level. Within a group, the bars correspond to different setting on the reward function $R$, the robot-assumed soldier's behavior model $\hat{\pi}_b$, and the actual soldier's behavior model $\tilde{\pi}_b$.}
%   \label{fig:reward_trust_bar_comparison}
% \end{figure*}
% \subsubsection*{\textbf{Observation 1: High-ability robot results in high team performance and high trust.}} In  Figure~\ref{fig:a}, a comparison within the first 4 groups shows that if we increase the robot's threat-detection accuracy by changing $\kappa_2$ from 2 to 50, both the team performance and the final trust increase.

% \subsubsection*{\textbf{Observation 2: Trust-seeking reward does not harm team performance when the robot is trustworthy.}} Within each group, the $i+4$th condition is identical to the to the $i$th one except the reward function $R$ the trust-seeking reward $R_t$ instead of the the mission reward $R_m$, $i=1,2,3,4$. In the first 4 groups, where the initial trust is set to 0.67, when changing reward from $R_m$ to $R_t$, team performance almost keeps unchanged while the final trust increases; however, in the last 2 groups, where the initial trust is 0.33, there is a decrement in team performance, which can be thought of as a compensation for the increment in the trust. Therefore, if the robot starts in a high-trust state, then seeking trust will not harm the long-term team performance, while if it starts in a low-trust state, insisting to gain trust will cause the team performance to decrease.

% \subsubsection*{\textbf{Observation 3: Low initial trust does not lead to low team performance in the reverse psychology model.}} In the first condition in each group, both the robot's assumed soldier's behavior model $\hat{\pi}_b$ and the soldier's actual behavior $\tilde{\pi}_b$ are the reverse psychology model $\hat{\pi}^r_b$. Comparing the first conditions in the 2nd group and the 5th group shows that the team performance increases when the initial trust decreases from $(\alpha_1=100,\beta_1=50)$ to $(\alpha_1=50,\beta_1=100)$. This can be explained by the fact that both low-trust state and high-trust state have high values, however, a perceived failure has a larger impact on trust than a perceived success, and thus manipulating the human will let the robot reach a high-value state faster.


% % \subsubsection*{\textbf{Observation 4: Disuse behavior leads to better team performance when initial trust is high}}
% % Within each of the first 4 groups, the team performance is higher in the 2nd, 4th, 6th, and 8th conditions, where the actual trust behavior $\tilde{\pi}_b$ is set to the disuse behavior $\pi_b^d$, than the team performance in the other conditions, where the actual trust behavior $\tilde{\pi}_b$ is set to the reverse psychology behavior $\pi_b^d$. 



% % the team performance is always higher when the soldier's actual trust behavior model $\tilde{\pi}_b$ is the disuse model $\pi_b^d$ than , 

% % \section{Discussion}
% % 1. if $\hat{d}_k$ differ a lot from  $\tilde{d}_k$, and there is not many sites left the robot will manipulate the human\\
% % 2. if sensed model differs from the actual human behavior model.\\
% % 3. if the human's information is accurate, the value function in the disuse model is almost same value under different trust status\\
% % 4. compare task reward under different setting: 2X2x2 robot Sensed Human Model x actual Human Model X Objective\\
% % 5. comopare task performance for different kappa\\
% \section{Discussion and Conclusion}
% Recap of the result The simulation results show that 


% discussion



% limitation and future work: release assumptions; human subject experiment



% Some observations are drawn based on reasonable assumption, such as the robot and the human has the similar objective.
% Robot will not manipulate the Human in the Disuse Model  Figure~\ref{fig:c} shows that the robot will not manipulate the human if it assumes the soldier will completely ignore its recommendation. This is a consequence of endowing the soldier his own reasoning model. We note that trust still play a role under the disuse assumption.  

